The AI Hippocampus: How Far are We From Human Memory?

Memory plays a foundational role in augmenting the reasoning, adaptability, and contextual fidelity of modern Large Language Models and Multi-Modal LLMs. As these models transition from static predictors to interactive systems capable of continual learning and personalized inference, the incorporation of memory mechanisms has emerged as a central theme in their architectural and functional evolution. This survey presents a comprehensive and structured synthesis of memory in LLMs and MLLMs, organizing the literature into a cohesive taxonomy comprising implicit, explicit, and agentic memory paradigms. Specifically, the survey delineates three primary memory frameworks. Implicit memory refers to the knowledge embedded within the internal parameters of pre-trained transformers, encompassing their capacity for memorization, associative retrieval, and contextual reasoning. Recent work has explored methods to interpret, manipulate, and reconfigure this latent memory. Explicit memory involves external storage and retrieval components designed to augment model outputs with dynamic, queryable knowledge representations, such as textual corpora, dense vectors, and graph-based structures, thereby enabling scalable and updatable interaction with information sources. Agentic memory introduces persistent, temporally extended memory structures within autonomous agents, facilitating long-term planning, self-consistency, and collaborative behavior in multi-agent systems, with relevance to embodied and interactive AI. Extending beyond text, the survey examines the integration of memory within multi-modal settings, where coherence across vision, language, audio, and action modalities is essential. Key architectural advances, benchmark tasks, and open challenges are discussed, including issues related to memory capacity, alignment, factual consistency, and cross-system interoperability.

==> bks/llm_agent_bk/TBD <==
A Survey on the Memory Mechanism of Large Language Model based Agents

zeyu zhang new wechat survey

\begin{itemize}
    \item https://github.com/mikekelly/AgentK
    \item memgpt %记忆分级存储，主上下文用于处理当前信息，框架可以根据需要调用和添加外部存储
    \item Context and Time Sensitive Long-term Memory
    \item AriGraph: Learning Knowledge Graph World Models with Episodic Memory for LLM Agents
    \item memagent
    \item metagpt
    \item autogpt
    \item  \url{https://mp.weixin.qq.com/s/SgKruI2_r8NBi7l1zEnvrw}
\end{itemize}

\textbf{D. Misc}
\begin{itemize}
    \item AIOS %LLM作为OS的一层，听用户需求，调系统指令
    \item supermemory %“Build your own second brain.” 用户可以把喜欢的idea、网页、twitter收藏到这里，调用Mem0来存储，并与其对话，它会在必要时调用以前的记忆查询和调用
\end{itemize}

Embodied 放在哪？
Open-Ended Instructable Embodied Agents with Memory-Augmented Large Language Models\\
Jarvis-1

Benchmark就找到这一个，可以忽略?
Evaluating Very Long-Term Conversational Memory of LLM Agents




==> bks/llm_agent_bk/llm_agent.tex <==
\section{Inference with Agent Memory}

\jiaqi{llm agent, agent memory(babyagi, cameol??}
\subsection{System 1 and 2 of Agent Memories}

% https://mp.weixin.qq.com/mp/appmsgalbum?__biz=MzkxNjcyNTk2NA==&action=getalbum&album_id=3589369424701915145&scene=173&subscene=&sessionid=svr_cd765bc1cb6&enterid=1727091137&from_msgid=2247483908&from_itemidx=1&count=3&nolastread=1#wechat_redirect

% \begin{figure}[h]
% \centering
% \tikzset{
%     basic/.style  = {draw, text width=2cm, align=center, font=\sffamily, rectangle},
%     root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white,text width=8cm, rotate=90, font=\footnotesize},
%     dnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
%     dnode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize},
%     mnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.2cm, font=\footnotesize},
%     mnode_2/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
%     mnode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize}, 
%     snode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
%     snode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize},
%     tnode/.style = {basic, thin, align=left, fill=pink!60, text width=15em, align=center},
%     xnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=blue!20,text width=5cm,},
%     wnode/.style = {basic, thin, rounded corners=2pt, align=left, fill=white,text width=5.15cm, font=\footnotesize},
%     wnode_1/.style = {basic, thin, rounded corners=2pt, align=left, fill=white,text width=2.5cm, font=\footnotesize},
%     wnode_2/.style = {basic, thin, rounded corners=2pt, align=left, fill=white,text width=8cm, font=\footnotesize},
% }
% %
% \begin{forest} 
% for tree={
%     grow=east,
%     growth parent anchor=east,
%     parent anchor=east,
%     child anchor=west,
%     edge path={\noexpand\path[\forestoption{edge},->, >={latex}] 
%          (!u.parent anchor) -- +(5pt,0pt) |- (.child anchor)
%          \forestoption{edge label};}
% }
% % l sep is used for arrow distance
% [Agent Memory, mnode_1    
%     [Short-term Memory, mnode_2 
%         [Pipeline, mnode
%             [Knowledge injection, mnode_1
%                 [{
%                 TRIME~\cite{zhong2022training},
%                 }, wnode_1]]
%             [Long contexts, mnode_1
%                 [{
%                 MemTRM~\cite{wu2022memorizing},
%                 }, wnode_1]]
%         ]
%         [System, mnode
%             [Finetuning, mnode_1
%                 [{
%                 RAG~\cite{NEURIPS2020_RAG},
%                 }, wnode_1]]
%              [Pretraining, mnode_1
%                 [{
%                 REALM~\cite{guu2020REALM},
%                 }, wnode_1]]
%         ]
%     ]
%     [Long-term Memory , mnode_2
%         [Pipeline, mnode
%             [{
%             LlamaIndex~\citep{Liu_LlamaIndex_2022}, 
%             LangChain~\cite{Chase_LangChain_2022}
%             },wnode]]
%         [System, mnode
%            [{
%            G-Retriever~\cite{he2024g},
%            },wnode]]
%         ]
%     ]
% ]
% \end{forest}

% \caption{Taxonomy of the structure design for learning with explicit memory.}
% \label{fig:taxonomy_efficient_structure}
% \end{figure}


\begin{figure}[h]
\centering
\tikzset{
    basic/.style  = {draw, text width=2cm, align=center, font=\sffamily, rectangle},
    root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white,text width=8cm, rotate=90, font=\footnotesize},
    dnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
    dnode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize},
    mnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.2cm, font=\footnotesize},
    mnode_2/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
    mnode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize}, 
    snode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
    snode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize},
    tnode/.style = {basic, thin, align=left, fill=pink!60, text width=15em, align=center},
    xnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=blue!20,text width=5cm,},
    wnode/.style = {basic, thin, rounded corners=2pt, align=left, fill=white,text width=5.15cm, font=\footnotesize},
    wnode_1/.style = {basic, thin, rounded corners=2pt, align=left, fill=white,text width=2.5cm, font=\footnotesize},
    wnode_2/.style = {basic, thin, rounded corners=2pt, align=left, fill=white,text width=8cm, font=\footnotesize},
}

\begin{forest}
for tree={
    grow=east,
    growth parent anchor=east,
    parent anchor=east,
    child anchor=west,
    edge path={\noexpand\path[\forestoption{edge},->, >={latex}] 
         (!u.parent anchor) -- +(5pt,0pt) |- (.child anchor)
         \forestoption{edge label};}
}
[LLM Memory Tools, mnode_1    
    [Integrating External Data Sources, mnode_2
        [LlamaIndex
            [Enhances response quality via retrieval systems]
        ]
        [MemGPT
            [Multi-agent multi-user deployment]
            [Supports custom tools]
        ]
        [LangChain
            [Modular framework]
            [Integrates models and data sources]
        ]
        [ModelScope\_agent
            [Extensive tools and APIs]
            [Supports various data types]
        ]
    ]
    [Efficient Memory Management and Retrieval, mnode_2
        [Mem0
            [Optimizes data access for large-scale LLMs]
        ]
        [Memary
            [Scalable memory systems]
            [Efficient data retrieval]
        ]
        [RedCache-AI
            [Advanced caching and retrieval]
            [Reduces latency]
        ]
    ]
    % [Graph-based Retrieval, mnode_2
    %     [GraphRAG
    %         [Leverages graph structures]
    %         [Improves response relevance]
    %     ]
    % ]
    [Deployment and Development Frameworks, mnode_2
        [LangChain
            [Short-term Memory: ConversationalBuffer]
            [Long-term Memory: Knowledge bases and persistent storage]
        ]
        [ModelScope\_agent
            [Tools and APIs for managing LLMs]
            [Supports various data input forms]
        ]
        [MemGPT
            [Flexible deployment options]
            [Run locally]
        ]
    ]
]
\end{forest}

\caption{How to choose the tools of memory.}
\label{fig:Tool_choose}
\end{figure}




Memory is the process used to acquire, store, retain, and subsequently retrieve information. In human brain, there are three main types of memories.
\jiaqi{references below}
 
\begin{itemize}
    \item \textbf{Sensory Memory}: The earliest stage of memory, which retains sensory information and includes Iconic (visual) Memory, Echoic (auditory) Memory and Haptic (touch) Memory.
    
    \item \textbf{Short-term Memory (STM)}: STM temporarily stores all the information currently in awareness, as well as information needed for complex cognitive tasks (such as learning and reasoning). \jiaqi{footnote, Typically stores 7 items, lasting about 20-30 seconds.}
    
    \item \textbf{Long-term Memory (LTM)}: LTM stores information for long periods, ranging from days to decades, with virtually unlimited capacity. One type of LTM is declarative memory of facts and events, which can be consciously recalled. Another type is procedural memory which is unconscious including skills like riding a bike or typing on a keyboard.
\end{itemize}

\newtcolorbox{definitionbox}{
  colback=blue!5!white,  % 背景颜色
  colframe=blue!75!black, % 边框颜色
  fonttitle=\bfseries,   % 标题字体
  title=Definition,      % 标题内容
  sharp corners,         % 边角设为直角
  boxrule=1pt,           % 边框宽度
}


Similar to how memory functions in human cognition, memory modules in LLM agents act as the "brain," enabling the accumulation of experience, continuous adaptation, and more consistent, rational, and effective behavior. The design of memory structures for these agents is inspired by the characteristics of human memory. In this context, we categorize LLM agents' memories into short-term and long-term components:

\begin{definitionbox}
\textbf{Short-term memory} refers to in-context learning, which is bounded by the limited context window of the Transformer architecture.

\textbf{Long-term memory} serves as an external storage system, accessible by the agent during queries through efficient retrieval mechanisms.
\end{definitionbox}


\input{sections/llm_agent/rag}




\subsection{System architechture}


% \textbf{B. Frameworks Specializing in Retrieval-Augmented Generation (RAG)}
\jiaqi{Comparison in Xmind}






\begin{itemize}
    \item \textbf{LlamaIndex}~\citep{Liu_LlamaIndex_2022} specializes in integrating LLMs with retrieval systems to enhance the quality of generated responses by leveraging external data sources. It uses indices and databases to store and manage retrieval-augmented content and supports data input forms of text, documents and knowledge bases. 
    
    \item \textbf{Mem0} focuses on efficient memory management and retrieval for large-scale LLMs, optimizing data access and integration. It implemented a specialized memory management system that supports both in-memory and disk-based storage and supports data input forms of text, documents and knowledge bases. 
    
    \item \textbf{RedCache-AI} provides advanced caching and retrieval solutions to enhance the performance of LLMs by reducing latency and improving access to stored data.
    RedCache-AI uses a combination of in-memory caches and persistent storage systems and supports data input forms of text, databases, structured data.
    
    \item \textbf{Memary} focuses on building scalable memory systems for LLMs, with an emphasis on efficient data retrieval and integration. It uses both in-memory and distributed storage solutions for flexibility and scalability and supports data input forms of text, documents, and knowledge bases.

    \item \textbf{GraphRAG} integrates graph-based retrieval with LLMs to improve the relevance and contextuality of generated responses by leveraging graph structures.
   It employs graph databases and indexing systems to manage memory and supported data input forms of Text, graphs, structured data.

    \item \textbf{MemGPT}~\citep{packer2023memgpt} features the ability to connect with external data sources, and support for integrating custom tools. It's designed for multi-agent, multi-user service deployment and is actively developed with a community that contributes to its ongoing improvement. MemGPT also provides extensive documentation and research backing, and it can be run locally for flexible deployment options.

\end{itemize}

\jiaqi{Summarize in one paragraph, footnote}

% \textbf{A. Comprehensive Agent}
\begin{itemize}
    % \item \textbf{LangChain}~\citep{Chase_LangChain_2022} presents a modular framework tailored for constructing LLM-powered applications. It streamlines the process by integrating with various LLMs, data sources, and tools, thereby easing the development of intricate applications. Depending on the integration, LangChain employs diverse storage mechanisms, enabling memory storage in databases, files, or cloud services. LangChain supports input forms such as text, documents, APIs, and databases.
    
    % The ConversationalBuffer in LangChain serves as a short-term memory component, offering quick access to recent conversational context for immediate response generation. It excels in resource efficiency, context sensitivity, and ease of updating. However, it faces limitations such as capacity constraints, transient nature, dependency on context, lack of broad knowledge, and difficulty in complex reasoning. Integrating short-term memory with long-term mechanisms is crucial for handling diverse conversational needs effectively.

    % LangChain addresses long-term memory through integration with external knowledge bases, persistent storage solutions, and memory networks that simulate the storage and retrieval of information. It includes mechanisms for memory retrieval based on contextual cues, context management, and updates. Tools for memory traceability and explainability are provided to enhance model transparency. The system also focuses on encoding and decoding, optimization for efficiency, security and privacy, and scalability to manage growing data. LangChain's approach to long-term memory is dynamic and evolves with the project's development, necessitating regular consultation of its documentation for the latest practices.


   \item \textbf{LangChain}~\citep{Chase_LangChain_2022} is a modular framework designed for building LLM-powered applications by integrating with various models, data sources, and tools. It supports diverse input forms (e.g., text, documents, APIs, and databases) and offers both short-term and long-term memory mechanisms. The ConversationalBuffer provides efficient, context-sensitive short-term memory but is limited by its capacity and inability to handle complex reasoning. For long-term memory, LangChain leverages external knowledge bases, persistent storage, and memory networks, providing tools for memory traceability, optimization, and scalability. Its long-term memory strategies are dynamic, requiring regular updates from documentation.
   
   \item \textbf{ModelScope\_agent}~\citep{li2023modelscope} is dedicated to providing an extensive array of tools and APIs for the management and deployment of LLMs. It seamlessly integrates with multiple data sources and offers various features crucial for application development.  ModelScope\_agent utilizes both in-memory and persistent storage solutions, allowing for adaptable memory management. It accommodates various data input forms including text, images, video, and structured data.
   %\item \textbf{CrewAI}
\end{itemize}


\textbf{Comparison of different tools}\\
Here we provide a comparison of different attributes of the tools in Table~\ref{tab:tool_attr}

\begin{table}[h]
\centering
\begin{tabular}{l|>{\centering\arraybackslash}p{2.5cm}|>{\centering\arraybackslash}p{2.5cm}|>{\centering\arraybackslash}p{2.5cm}|>{\centering\arraybackslash}p{2.5cm}|>{\centering\arraybackslash}p{2.5cm}}
\toprule
\textbf{Tool} & \textbf{Data Sources} & \textbf{Database Type} & \textbf{Indexing and Retrieval Methods} & \textbf{Application Scenarios} & \textbf{User Interface} \\
\midrule
LangChain Memory & Text input from user interactions; conversation history & Memory variables; expandable to external storage (e.g., databases, Redis) & Sequential storage of conversation turns; context management; advanced retrieval using embeddings & Chatbots; conversational agents that need to maintain context & Python classes and methods provided by LangChain \\
\midrule
ModelScope Agent Memory & Text input; supports multimodal data & In-memory storage; supports external databases & Retrieval using embeddings; advanced memory retrieval methods & AI assistants, chatbots, multimodal applications & APIs and tools provided by ModelScope \\
\midrule
LlamaIndex & Text documents, PDFs, images, etc. & Vector databases (e.g., FAISS, Pinecone) & Index data using embeddings; retrieve via similarity search & Knowledge base Q\&A, document search, chatbots with external data access & Provides Python APIs and tools; integrates with LLMs \\
\midrule
Mem0 & Text input, conversation history, personal documents & Vector databases or similar storage & Uses embeddings and similarity search & Personal AI assistants with memory, knowledge management & Provided APIs and tools; integration via SDK \\
\midrule
GraphRAG & Structured data, knowledge graphs & Graph databases (e.g., Neo4j) & Graph traversal; querying through graphs & Complex reasoning tasks; applications leveraging structured knowledge & APIs of graph databases; query languages like Cypher \\
\midrule
MemGPT & Text input, conversation history & External memory modules; databases or in-memory storage & Customized memory mechanisms; may use embeddings & Conversational agents requiring long-term memory & Depends on implementation; provides APIs or code examples \\
\bottomrule
\end{tabular}
\caption{Comparison of LLM Agent Memory Tools}
\label{tab:tool_attr}
\end{table}


==> bks/llm_agent_bk/rag.tex <==
\subsection{Single-agent Memory} 
%Agent workflow memory
Recently, more studies augment \ac{llm} agent with the non-parametric external memory \citep{mai2023llm, maharana2024evaluating, yang2024memory3}. It enhances the agent's ability to explicitly store, retrieve, and utilize memory for various tasks. These works generally have two key stages: (1) recalling relevant thoughts from memory before generating a response and (2) post-thinking after generating a response to incorporate both historical and new thoughts into memory, thus improving consistency and efficiency.
% avoiding inconsistencies and inefficiencies. %通过维护和更新一个llm外挂的memory, 大量交互历史traj和学习的新知识可以被更好的抽取和利用, 可以在inference用有什么好处, 有助于持续学习 %参考ram
In this section, we synthesize a wealth of research dedicated to leveraging external memory using refined and optimized RAG methods at inference time for the LLM agent on better downstream tasks.
\subsubsection{Short-term Memory}
Short-term memory serves as a transient storage system within LLMs; it is typically implemented by maintaining recent inputs within the context window of LLMs. Due to the limited length of the context window, history inputs before a time point will be discarded inevitably. Nevertheless, short-term memory improves the continuity and consistency of LLM and benefits LLMs in many challenging tasks that involve multi-hop reasoning and sequential decision-making.



\textbf{Chain-of-Thought (CoT)}~\citep{wei2022chain} prompting explicitly asks LLMs to generate intermediate reasoning steps that lead to the final answer. The intermediate reasoning steps (aka. thoughts) are stored in the context of LLMs, act as their working memory, and stimulate their logical reasoning.
Differently from CoT, where reasoning follows a linear-chain structure, \textbf{Tree of Thoughts (ToT)}~\citep{yao2024tree} prompting solves problems by considering multiple different reasoning paths defined on a tree structure. The tree-structured reasoning allows for efficient forward-looking and backward-tracking, two crucial aspects of advanced search-based problem solvers.
Generalizing CoT and ToT, \textbf{Graph of Thoughts (GoT)}~\citep{besta2024graph} prompting enables reasoning over a graph structure, where each node represents an intermediate thought and the edges encode the dependency between the thoughts. GoT is a more flexible prompting paradigm since it allows for a wide range of thinking transformations, e.g., it is convenient to aggregate thoughts and switch between different reasoning flows on a graph structure.

% enabling it to better simulate human thought processes. It uses units of LLM thoughts as vertices and dependencies between these vertices as edges to combine arbitrary LLM thoughts and extract the essence of the entire thought network. It support a variety of thinking transformations such as aggregating, generating especially in scenarios where multiple solutions need to be synthesized or the reasoning flow changed as new insights are discovered.

%COT-SC


\textbf{ReAct}~\citep{yao2022react} is a novel approach that prompts LLMs to generate both reasoning traces and task-specific actions in an interleaved manner, fostering synergy between the two processes. This method combines reasoning and acting of LLM and allows the model to dynamically update action plans through reasoning and interact with external sources like Wikipedia to enhance decision-making.

% \paragraph{Reflection}
%textgrad
%self-reflection

\paragraph{Reflexion}~\citep{shinn2024reflexion} builds uponReAct and enhances the decision-making ability of LLMs using verbal reinforcement learning. At the core of Reflexion is deliberate reflection on natural language feedbacks obtained from task outcomes, rather than through weight updates. Reflexion firstly explores the property of self-reflection in LLMs and shows that self-reflection is extremely useful to iteratively learn over trials as another form of short-term memory. Similar to Reflexion, which leverages linguistic feedback, \citet{gupta2024metareflection} learns general prompt instructions for LLMs using past self-reflections. Specifically, it gathers self-reflections in training and generalizes them into verbal 'meta-reflections' which serve as additional instructions to enhance the efficiency of agent's. 
RefAug~\citep{zhang2024learn} uses reflective augmentation to embed reflective sections within training instances, encouraging models to consider alternative solutions and engaging in deeper reasoning. Notably, This method goes beyond standard data augmentation by fostering a more comprehensive understanding of mathematical problems. 
Reflection on search Trees (RoT)~\citep{hui2024rot} is introduced to reflect on an LLM's previous tree search experiences to generate guidelines, which are then used to improve the model's decisions in subsequent searches. This approach prevents repeated mistakes and enhances search efficiency. A key innovation is the identification of critical information from historical searches to produce more effective guidelines. Mirror~\citep{yan2024mirror} is a multiple-perspective self-reflection method to addresses the limitations of LLMs in self-assessment and feedback generation by introducing a Navigator-Reasoner framework. It improves through a heuristic interaction between a navigator, which provides question-adaptive directions, and a reasoner, which assesses and refines predictions based on the directions from the navigator. 



% \end{itemize}

\subsubsection{Long-term Memory}

While operating in a real-time environment, crucial information, interactive feedback and distilled experience need to be continuously collected and further extracted from short-term memory and preserved as long-term memory of the LLM agent for future reference. To provide the agent with useful knowledge and experience for latter use, some works~\citep{huang2024understanding, park2023generative, wang2023recmind, zhang2024large} incorporate long-term memory (LTM) to LLMs from both user-specific and common-sense perspectives. This enables LLMs to flexibly utilize past experiences in accordance with current situations and enhance their task-planning and decision-making capabilities. These works usually formulate and organize thoughts in memory based on operations like insert, forget, merge and others, enabling dynamic updates and evolution of the memory in the long run. 

In this section, we mainly discuss four typical categories of long-term memory for a LLM agent as below:
% 1. **Knowledge Base Integration**: Some frameworks extend their long-term memory by integrating with external knowledge bases that may contain a wealth of structured or semi-structured data.
% 2. **Persistent Storage**: Long-term memory may involve storing information in databases or file systems for access beyond the model's session.
% 3. **Memory Networks**: Certain frameworks might employ memory network technology, simulating human long-term memory with an external storage component that aids in retrieving and utilizing stored information when needed.
% 4. **Memory Retrieval and Updating**: Effective long-term memory management includes mechanisms for memory retrieval and regular updates to reflect new learning outcomes and information.
% 5. **Scalability**: As the volume of data grows, long-term memory mechanisms need to be scalable to handle and store more information.
% 6. **Security and Privacy**: Ensuring the security and privacy of data is crucial when dealing with long-term memory, especially when sensitive information is involved.
% \textbf{Integrated Application}
% - **Complementary Strengths**: Short-term and long-term memory in LLM frameworks typically need to complement each other, with short-term memory handling immediate conversational needs and long-term memory providing broader background knowledge and persistent information storage.
% - **Dynamic Balancing**: Models need to find a balance between the quick responsiveness of short-term memory and the depth of knowledge from long-term memory to adapt to different conversational scenarios and task requirements.
% Different LLM frameworks may employ various technologies to implement these memory mechanisms, such as specific algorithm optimizations, hardware acceleration, or software architecture designs. For details on the implementation of a specific framework, it is recommended to consult relevant technical documentation or research papers.


% \begin{table}[t]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|ccccccc}
%     \toprule
%         Title & Memory source & Memory data type & Memory granularity  & Stage \\  
%     \midrule
%         DynaMind & Previous interactions,  External databases, 
% Internet &Text &Triple  &Inference   \\
%         RET-LLM & Not mentioned  &Text &Triple  &Inference  \\
%         HAT  &History conversation sessions &Text  &Tree node  &Inference  \\
%         COMEDY & History conversation summaries  %(events, user/bot portraits, user-bot relations) 
%         &Text  &Sentences  &Inference  \\
%         TiM & Previous trajectories &Text  &Sentences   &Inference  \\
%         LOCOMO & History conversation summaries, observations, reflections &Text  &Sentences   &Inference  \\
%         RAP & Previous trajectories &Text, Vision  &Sentences, Image   &Inference  \\
%         Learning to Repair & Feedback &Text &Sentences   &Inference  \\
%         MemPrompt & Feedback &Text &Sentences   &Inference  \\
%         TeachMe & Feedback &Text &Sentences   &Inference  \\
%         KnowledGPT & Wikipedia, CN-DBPedia,
% personalized documents &KG &Sub-Graph   &Inference  \\
%         DPeM & History conversation, summaries &Text &Sentences   &Inference  \\
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{10pt}
%     \caption{Summarization of inference with explicit memory}
%     \label{tab:benchmark}
% \end{table}

% \textbf{A. Pre-retrieval}

% 1. index-structure
% \begin{itemize}

    
%     \item \textbf{ISEEQ} is a conversational information retrieval method designed to autonomously formulate Information Seeking Questions (ISQs) from succinct user inquiries. This innovative system is comprised of three sophisticated components: the Semantic Query Expander (SQE), which enhances the semantic richness of queries; the Knowledge-aware Passage Retriever (KPR), designed to leverage knowledge graphs for bolstering unsupervised passage retrieval; and the generative adversarial reinforcement learning-based question-answering generation model, known as ISEEQ-RL.
    
%     \item \textbf{G-Retriever} combines the strengths of GNNs, LLMs, and RAG to propose a method for enhancing graph understanding. The retrieval-augmented generation in this framework is typically implemented through four steps: indexing, retrieval, subgraph construction, and generation. During the indexing phase, nodes and edges are generated by a pre-trained language model and stored in a nearest neighbor data structure. Then, the k-nearest neighbors method is used to retrieve the nodes and edges most relevant to the query. For these nodes and edges, subgraph construction employs the Prize-Collecting Steiner Tree algorithm to build a subgraph that includes as many relevant nodes and edges as possible while keeping the graph size manageable. Finally, an answer is generated using an "graph prompt," a textualized graph, and the query through the LLM.
    
%     \item \textbf{KGP} introduces an innovative approach to knowledge graph prompting, adeptly crafting the ideal context for LLMs by constructing and navigating through a knowledge graph that encompasses a multiple documents, thereby improving the performance of multi-document question answering. For graph constraction, nodes and edges are constructed by analyzing the semantic/lexical similarity between passages or document structural relations.Central to its retrieval prowess is the design of an LLM-driven graph traversal agent. This agent adeptly evaluates the similarity between prospective neighboring sentences and the passages generated, ensuring that only the most contextually pertinent nodes are selected to advance to the subsequent traversal phase.
% \end{itemize}

% 2. query optimization
% \begin{itemize}
%     \item \textbf{Trainable rewriter}~\citep{Ma2023QueryRF} In order to enhance the consistency between the retrieved knowledge and the input text, this paper proposes a new framework called "Rewrite-Retrieve-Read," which introduces a query rewriting step in LLMs. The core of the method lies in the introduction of a small trainable rewriter, which is further trained using reinforcement learning, taking the output of the LLMs as a reward signal. Additionally, it utilizes a web search engine as the retriever to search for relevant documents based on the rewritten queries. The advantage is that it can access the most up-to-date knowledge without the need to store or maintain a knowledge base.
% \end{itemize}

% \textbf{B. Post-retrieval}

% 1. rerank chunks

% 2. context compressing
% \begin{itemize}
%     \item \textbf{PRCA}~\citep{yang-etal-2023-prca} is a trainable Pluggable Reward-Driven Contextual Adapter, consisting of a contextual extraction phase and a reward-driven phase, capable of effectively distilling retrieved information and enhancing the performance of generators in ReQA tasks. PRCA initially extracts textual information from the retrieved TOP-K relevant documents, refining an output sequence that minimizes the difference from the true context. The goal of the reward-driven phase is to align the contextual output sequence with the downstream generator, optimizing the retrieved information through the generator's rewards so that it can effectively guide the generation of answers. This method not only improves the efficiency of the generator but also simplifies the generator's processing by reducing the length of the input text.
    
%     \item \textbf{DPR}~\citep{karpukhin-etal-2020-dense} introduces an innovative dense passage retrieval method that surpasses traditional models in semantic understanding. This approach is underpinned by a dual-encoder architecture, comprising a question encoder and a passage encoder that operate independently. The method refines embedding representations by training on positive and negative examples, ensuring closer vector alignment for relevant content, thus improving retrieval accuracy. In the inference stage, passages are encoded and indexed, enabling the retrieval of the top k passages that bear the highest similarity to the question vector, facilitated by the maximum inner product search algorithm. Moreover, the FAISS library is used for efficient vector indexing, enhancing open-domain QA system performance.

%     \item \textbf{RECOMP} framework enhances language model efficiency and performance by compressing retrieved documents into concise textual summaries prior to ingestion. This system incorporates two types of compressors: the extractive compressor, which identifies and selects pertinent sentences from the retrieved documents, and the abstractive compressor, which creates summaries by amalgamating information across various documents. To refine the summarization process, RECOMP introduces a training regimen that leverages end-task indicators from the language model, enabling the compressor to execute selective augmentation and ensure the summaries are both effective and succinct.
% \end{itemize}

% \textbf{C. Flexible retrieval}


% \item \textbf{Interleaving Retrieval}~\citep{trivedi2022interleaving} introduces a novel approach for few-shot multi-step open-domain QA that integrates retrieval with chain-of-thought reasoning to enhance the performance of knowledge-intensive QA.
% It alternates between extending the chain-of-thought and retrieving additional information, using the evolving reasoning to guide the retrieval process, which in turn refines the reasoning.

% \item \textbf{TOC}~\citep{kim2023tree} is designed to handle ambiguous questions in open-domain QA by generating comprehensive long-form answers without requiring user clarification. TOC recursively constructs a tree of disambiguations for an ambiguous question using retrieval-augmented clarification, leveraging external knowledge sources to explore multiple dimensions of ambiguity with a self-verification pruning.

% \item \textbf{FLARE}~\citep{jiang2023active} dynamically actively decides when and what information to retrieve during the text generation process. FLARE iteratively generates a temporary next sentence, uses it as a query to retrieve relevant documents if it contains low-confidence tokens, and regenerates the sentence. It avoids unnecessary or inappropriate retrieval and improves the efficiency of information gathering.


\paragraph{Memory of fact knowledge}

The vast number of parameters in \ac{llm} endows them with remarkable capabilities, allowing them to excel in a variety of \ac{nlp} tasks. However, this complexity also presents challenges, making LLMs difficult to train and inhibiting their ability to continuously assimilate new knowledge\citep{zhang2023large}, which may lead to inaccuracies in their outputs. 
In order to resolve these issues, \citet{du2023static} propose a continual learning framework that incorporates memory mechanisms allowing LLMs to assimilate new knowledge and modular operators to enhance model inference with this newly acquired knowledge. DynaMind is designed to enabling LLM to dynamically adapt to evolving environments and continuously integrate new information without the need for parameter tuning. Similarly, \citet{modarressi2023ret} augments \ac{llm} with a write-read memory module by extracting and saving knowledge in the form of triplets, allowing for scalable, updatable, interpretable, and aggregatable memory storage, which is particularly beneficial for handling temporal-based question answering tasks. 


\paragraph{Memory of historical trajectories and experience}

Incorporating memory into agents is crucial for enhancing their ability to remember historical trajectories, which ultimately improves decision-making and learning efficiency. By allowing agents to recall past experiences, they can identify patterns, make more informed predictions, and adapt their strategies based on historical data. This memory mechanism enables agents to build upon previous knowledge, facilitating more nuanced and contextually relevant responses. Delving into the integration of memory also supports the development of more sophisticated models that parallel the cognitive processes of humans, thereby advancing the overall effectiveness and versatility of artificial intelligence systems.
\citet{guo2023empowering} incorporate a centralized working memory hub and episodic buffer access to retain memories across episodes. This architecture aims to provide greater continuity for nuanced contextual reasoning in intricate tasks and collaborative scenarios. \citet{liu2023think} also maintains an evolved memory for storing historical thoughts and employs Locality-Sensitive Hashing for efficient retrieval. \citet{kagaya2024rap} introduces Retrieval-Augmented Planning (RAP) with a contextual memory module to leverage past experiences for improved decision-making in complex tasks. RAP dynamically retrieves relevant past experiences based on current context to guide planning and action selection, mirroring human-like analogical reasoning.

\paragraph{Memory of user feedback}

Recently, many researchers have proposed various methods for \ac{llm} to continue to improve without retraining. The \ac{lm} is coupled with a growing memory module with feedback either corrections on the historical errors or better clarifications on the tasks from the users. \citet{madaan2022memory} maintains a growing memory of misinterpretation of user intents, along with user feedback for clarification. This memory enables the system to produce enhanced prompts for new queries based on past user feedback, effectively leveraging previous corrections to improve performance on similar tasks.  \citet{tandon2021learning} enables \ac{llm}'s to improve their output after deployment without retraining, by leveraging user feedback. It maintains a dynamic memory of cases where users have identified and corrected output errors, and uses a trained corrector model to apply similar feedback to fix new errors. This approach shows significant improvement in repairing errors and avoiding past mistakes on new examples. The system represents a step towards continuous model enhancement through interactive learning and memory-based feedback reuse. \citet{dalvi2022towards} integrates a dynamic memory component that stores user-provided corrections to the model's erroneous beliefs. These corrections are retrieved and used as additional context when answering new questions, helping the system avoid repeating past mistakes. This approach represents a novel application of memory-based continual learning for belief maintenance in language models, allowing for user-driven system enhancement over time. In order to maintain an ever-improving memory for \ac{llm},  \citet{li2024ram} utilizes recursive reasoning-based retrieval and experience reflections to continually update the memory and learn from communicative feedback provided by users. Without periodically re-training, it enables \ac{llm} to obtain fresh knowledge and historical experience by dynamically improving and growing a continually updated memory through human communications.
%In order to learn the ever-changing knowledge in the world for LLM, \citet{li2024rameverimprovingmemorylearning} introduces an innovative RAG-based framework with an ever-improving memory called RAM. Inspired by humans'pedagogical process, RAM utilizes recursively reasoning-based retrieval and experience reflections to continually update the memory and learn from users' communicative feedback through communicative learning.

% \item \textbf{MQUAKE}~\citep{zhong2305mquake} introduces a benchmark for assessing knowledge editing in language models, focusing on multi-hop questions that require models to answer questions with answers that change as a consequence of edited facts. The authors also propose MeLLo, a memory-based approach that stores edited facts externally and prompts the language model iteratively to generate answers consistent with the edited facts. 

\paragraph{Memory of dialogues and personalized configuration}
To address the limitation of context capacity over long conversations, \citet{aadhithya2024enhancing} introduces a novel memory structure that recursively aggregates dialogue context flexibly to enhance long-term memory for dialogue agents. It allows for broad coverage of information with controlled depth through conditional tree traversals, balancing the breadth and depth of information for long-form dialogues, which is crucial for multi-turn reasoning without exponential parameter growth.  Based on this,  \citet{chen2024compressimpressunleashingpotential} adopts compressive memory that integrates session-specific summaries, user-bot dynamics, and past events into a concise memory format. This method is designed to be more manageable and efficient than traditional retrieval-based methods using \ac{dpo} to enhance the model's ability to generate contextually appropriate responses. In \citet{maharana2024evaluating}, memory in these papers contains more nuanced and human-like conversational experiences, showing its effectiveness in managing time-dependent information and maintaining coherence in long-term and varied interactions, significantly contributing to the field of conversational agent. 

Incorporating personalized knowledge bases into memory allows users to effectively store and access specific knowledge according to their requirements.
\citet{wang2023knowledgpt}  is a novel framework for knowledge retrieval and personalized knowledge base interaction. It employs the ``Program of Thoughts'' (PoT) prompting method, which facilitates model interaction with Knowledge Bases through the generation of Python code, thereby enabling knowledge retrieval.  For domain specific tasks, \citet{zhang2023memory} introduces a personalized medical assistant tasks through a computational bionic memory. It utilizes a memory generation module using Dual-Process enhanced Memory (DPeM) that fine-tunes the LLM to produce personalized responses. ~\citet{zhong2024memorybank} enables storing past conversations and adapting to user personalities. The system is showcased through SiliconFriend, a chatbot that provides empathetic and long-term companionship, demonstrating MemoryBank's effectiveness in improving AI engagement.

 



\subsection{Multi-agent Memory}
\begin{itemize}
    \item \textbf{Memory Sharing}~\citep{gao2024memory} discusses the concept of memory sharing in the context of LLM-based agents, focusing on the importance of working memory in enhancing agent capabilities. The paper explores how agents can share memories to improve performance in multi-agent systems.
    \item \textbf{TaskGen}~\citep{tan2024taskgen} introduces an open-source framework that employs agents to break down tasks into subtasks executable by Equipped Functions or other agents. It utilizes StrictJSON for concise, type-checked JSON output from LLMs, optimizing token usage and processing efficiency. It features a shared memory system that manages information flow based on the need-to-know principle and showcases capabilities through various tasks, achieving high solve rates in dynamic environments and complex problem-solving.
    \item \textbf{SMART}~\citep{kannan2023smart} proposes a framework for multi-robot task planning leveraging LLMs to interpret high-level instructions and generate task plans and implements stages of task decomposition, coalition formation, and task allocation using a real-time memory storage and retrieval mechanism. The memory pool is dynamically updated through interactions among multiple agents to enhance task planning capabilities. It also introduces a benchmark dataset for evaluating multi-robot task planning with varied complexity levels and demonstrates the framework's effectiveness through simulations and real-world robot experiments.
    \item \textbf{Internet of Agents}~\citep{chen2024internet} has a specific data Layer which functions as the agent’s memory. The data layer maintains local data relevant to the agent’s operations. It includes the Agent Contact Block for storing information about other agents the current agent has interacted with, the Group Info Block for maintaining details about ongoing group chats and collaborations, and the Task Management Block for tracking the status and progress of tasks assigned to the agent.

\end{itemize}


==> bks/mllm/mllm_memory.tex <==
\section{Memory-augmented Multi-Modal Large Language models}\label{sec:mmllm}

This reading list is composed of two comprehensive parts:

\textbf{Multimodal Context Modeling with Memory}: This section explores how memory mechanisms are employed to model and retain long-term contextual information across various modalities, such as audio and video. It covers techniques for enhancing the understanding and processing of continuous and complex multimodal data.

\textbf{Multimodal Contextual Memory for Vision and Robotics}: This part focuses on the integration of memory mechanisms to augment the capabilities of embodied agents and robotics. It includes applications such as long-term planning, decision-making, visual navigation, and manipulation reasoning, demonstrating how memory can significantly enhance an agent's ability to operate in complex environments.


% \textbf{External Multimodal Knowledge/Memory Augmentation}: Here, we delve into the use of memory as an external knowledge source. This external information serves as complementary data that can enhance the performance and capabilities of models by providing additional context and insights, thereby improving their overall effectiveness.




\subsection{Multimodal Context Modeling with Memory}

In this section, we introduce the multimodal context modeling with memory, incorporating information from audio, video, and other modalities. For each modality, we will discuss its modeling in relation to various downstream tasks.




\subsubsection{Audio Context  Modeling}


The continuous and high-frequency nature of audio presents significant challenges in efficiently modeling its sequences, demanding substantial computational resources. As a result, developing effective methods to incorporate audio history is crucial for various applications. Recent advancements in audio context modeling have introduced innovative solutions to address these challenges. For instance, Conformer-NTM \cite{DBLP:conf/interspeech/CarvalhoA23} proposes an external memory network between the encoder and decoder transformers for automatic speech recognition (ASR), enhancing the system's ability to handle complex audio sequences. Similarly, Loop-Copilot \cite{DBLP:journals/corr/abs-2310-12404} introduces a Global Attribute Table that identifies and manages various musical attributes at any moment, aiding in task execution and ensuring musical coherence in music generation. Furthermore, MR-MT3 \cite{DBLP:journals/corr/abs-2403-10024} employs previous instrumental tokens as key/value memory, effectively preventing instrument leakage in automatic music transcription tasks. These approaches demonstrate promising strategies for improving audio modeling, paving the way for more efficient and coherent audio processing systems.
% \begin{itemize}
%     \item Conformer-NTM\cite{DBLP:conf/interspeech/CarvalhoA23} porpose an external memory based on memory network between encoder-decoder transformer for ASR
%     \item Loop-Copilot\cite{DBLP:journals/corr/abs-2310-12404} propose Global Attribute Table for various attributes that define the musical piece at any given moment. which could facilitate task execution, and maintain musical coherence  for music generation
%     \item MR-MT3\cite{DBLP:journals/corr/abs-2403-10024} takes previous instrumental tokens as k/v memory to prevent from instrument leakage for automatic music transcription task.
% \end{itemize}

\subsubsection{Video Context Modeling}

Video context modeling presents unique challenges compared to image processing due to its added time dimension, which significantly increases complexity. Most existing approaches use sampling-based methods, converting continuous video into discrete stacked frames. This makes balancing computational complexity with detailed video information a crucial focus in video research. Memory mechanisms have emerged as a vital strategy in achieving this balance. This section explores various aspects of video context modeling, starting with general video representation learning, focusing on developing more effective video encoders. We then delve into recent advancements in memory mechanisms for large video language models and video agents, which demonstrate strong performance in zero-shot video-language benchmarks and applications. Finally, we discuss the role of memory in various downstream tasks.

\paragraph{Video Representation Learning}
In the realm of video representation, MC-ViT \cite{DBLP:journals/corr/abs-2402-05861} introduces a long video encoder using memory consolidation and cross-attention on video segments to efficiently encode long-context videos. This enhances the ability to handle extensive video data while maintaining detailed representation.

\paragraph{Large Video Language Models}

For large video language models, several innovative memory-augmented approaches have been developed for long video modeling. MovieChat \cite{DBLP:journals/corr/abs-2307-16449} builds on Q-Former for visual feature extraction with memory consolidation to model long videos for video question answering (QA). MA-LMM \cite{DBLP:journals/corr/abs-2404-05726} extends this with a retrieval strategy based on the semantic similarity of frame features. VideoStreaming \cite{DBLP:journals/corr/abs-2405-16009} proposes an method combined with an adaptive memory selection strategy on the recurrent image feature, selecting a constant number of question-related memories using Gumbel-Softmax. Flash-VStream \cite{DBLP:journals/corr/abs-2406-08085} presents a hierarchical memory system, incorporating FIFO queue for spatial features, and uses abstract memory implemented by cross-attention for whole video modeling. Additionally, OmniDrive \cite{wang2024omnidriveholisticllmagentframework} utilizes a memory bank for frames in autonomous driving-related QA.

\paragraph{Video Agent}
Video agents have made significant strides by transforming various video elements into text, such as captions, object names, and timestamps, which are then stored as external memory for LLMs to enhance video processing tasks. LLoVi \cite{DBLP:journals/corr/abs-2312-17235}, LifelongMemory \cite{DBLP:journals/corr/abs-2312-05269} and VideoAgent\cite{DBLP:journals/corr/abs-2403-10517} leverage captions as a memory for LLMs. Furthermore, VideoAgent \cite{DBLP:journals/corr/abs-2403-11481} combine captioning, tracking, VQA modules to inject video object detection ability into LLM. ChatVideo \cite{DBLP:journals/corr/abs-2304-14407} utilizes captioning, tracking, and audio modules to extract information from video as memory.  DoraemonGPT \cite{DBLP:journals/corr/abs-2401-08392} adopts a more comprehensive method by incorporating captioning, tracking, ASR, detection, action, and segmentation module to provide additional information for LLMs in video QA and segmentation tasks. LangRepo \cite{DBLP:journals/corr/abs-2403-14622} integrates captions, and timestamps as memory to LLMs for sequential understanding.  Finally, DrVideo \cite{DBLP:journals/corr/abs-2406-12846} reinterprets long-video understanding as a long-document comprehension task, effectively utilizing the power of large language models. These advancements underscore the diverse strategies employed to address the complexities of video context modeling and suggest promising directions for future research.


% \paragraph{Video Representation}
% \begin{itemize}
%     % general encoder
%     % transformer
%     \item MC-ViT\cite{DBLP:journals/corr/abs-2402-05861}; propose  Long video encoder vit, adopting memory consolidation + cross attention of video segment to encode long context video
% \end{itemize}


% \paragraph{Large Video Language Models}

% \begin{itemize}
%     \item MovieChat\cite{DBLP:journals/corr/abs-2307-16449} build on qformer with long term memory and memory consolidation to model long video for video qa 
%     \item MA-LMM\cite{DBLP:journals/corr/abs-2404-05726}; extend instructblip with qformer and retrieval strategy to consolidation by semantic similarity of frame feature to modeling long context video
%     \item VideoStreaming\cite{DBLP:journals/corr/abs-2405-16009}; further propose qformer + retrieval with Adaptive Memory Selection strategy selects a constant number of question-related memories from all the historical memories implemented by gumbel-softmax
%     \item Flash-VStream\cite{DBLP:journals/corr/abs-2406-08085}; present hierachical memory including spatial memory:FIFO, Temporal memory:Kmeans+topk, abstract memory: cross attention

%     % vertical application
%     \item OmniDrive\cite{wang2024omnidriveholisticllmagentframework}; memory bank for frame for Autonomous driving related QA
% \end{itemize}

% \paragraph{Video Agent}


% \begin{itemize}
%     \item ChatVideo\cite{DBLP:journals/corr/abs-2304-14407} propose caption + tracking + audio for videoQA
%     \item LLoVi\cite{DBLP:journals/corr/abs-2312-17235} caption + LLM for video QA
%     \item LifelongMemory\cite{DBLP:journals/corr/abs-2312-05269} caption + LLM for video QA
%     \item DoraemonGPT\cite{DBLP:journals/corr/abs-2401-08392} caption, track, asr, detect, action, segment + LLM for video QA/segment
%     \item LangRepo\cite{DBLP:journals/corr/abs-2403-14622} ChatGPT; caption + timestamp + LLM for video QA
%     \item VideoAgent\cite{DBLP:journals/corr/abs-2403-11481} caption + tracking + vqa + LLM for video QA
%     \item VideoAgent\cite{DBLP:journals/corr/abs-2403-10517}  caption + LLM for video QA
%     \item DrVideo\cite{DBLP:journals/corr/abs-2406-12846} convert the long-video understanding problem into a long-document understanding task so as to effectively leverage the power of large language model
% \end{itemize}



\paragraph{Downstream tasks -- overview}
In recent years, advancements in video understanding and generation have highlighted the critical role of memory mechanisms in enhancing long-context modeling capabilities. Researchers have been increasingly focused on developing innovative approaches to leverage these memory mechanisms across various video processing tasks. This survey provides an overview of these advancements, beginning with video understanding at the object level, progressing through action-level tasks, and culminating in general-level applications such as summarization, captioning, and question answering. Additionally, we explore recent breakthroughs in video generation that utilize memory-based architectures.


\paragraph{Downstream tasks -- object-level}

Object segmentation and tracking in videos are foundational tasks that benefit significantly from memory-augmented models. Early efforts in this domain employed RNNs, LSTMs, and GRUs to maintain and update memory states over time. For instance, ConvGRU \cite{DBLP:conf/iccv/TokmakovAS17} integrates convolutional gated recurrent units to track the evolution of objects within a scene, while RFL \cite{DBLP:conf/iccvw/YangC17} utilizes convolutional LSTMs for object tracking with preserving video instory. RMAN \cite{DBLP:journals/tip/PuSMZY21} builds on the LSTM architecture by adding a memory activation layer specifically for visual tracking.

Further advancements introduced more sophisticated memory networks. MemTrack \cite{DBLP:conf/eccv/YangC18} employs a dynamic memory network to store and recall target information, utilizing an LSTM to manage memory operations for template-matching tasks. STM \cite{DBLP:conf/iccv/OhLXK19} and its enhanced version, STCN \cite{DBLP:conf/nips/ChengTT21}, compute spatio-temporal attention across video frames, improving pixel-level object distinction. STMTrack \cite{DBLP:conf/cvpr/FuLFW21} introduces a mechanism that stores historical target information to guide the tracker toward the most informative regions.

Graph-based memory networks have also shown promise in video object segmentation. GraphMemVOS \cite{DBLP:conf/eccv/LuWDZSG20} leverages an episodic memory network structured as a fully connected graph, facilitating cross-frame correlation capture. DTMNet \cite{DBLP:conf/mm/ZhangWLL0L20} builds on this by incorporating both short- and long-term memory storage to enhance temporal modeling. TMRN \cite{DBLP:conf/iccv/SunWMZW23} improves memory retrieval operations by spatially aligning memory frames with current frames before temporal aggregation.

The advent of transformer-based architectures has further revolutionized object segmentation and tracking. AOT \cite{DBLP:conf/nips/YangWY21} employs long-short term memory for associating multiple object segments, while IMANet \cite{DBLP:conf/iros/PaulDGT21} utilizes attention mechanisms to access semantic information stored in memory. TrackFormer \cite{DBLP:conf/cvpr/MeinhardtKLF22} and XMem \cite{DBLP:conf/eccv/ChengS22} exemplify the integration of transformers with memory modules to handle occlusions and segment long video sequences effectively. Recent innovations continue to push the boundaries of memory utilization. S-ViT \cite{DBLP:conf/cvpr/ZhaoLTCCZ23} and MMC \cite{DBLP:journals/corr/abs-2307-07812} focus on preserving detailed feature maps and reducing background confusion through multiscale memory transformers. RFGM \cite{DBLP:conf/nips/ZhouGHL0GZ23} introduces a relevance attention mechanism to adaptively assist in selecting pertinent historical information. RMem \cite{DBLP:journals/corr/abs-2406-08476} enhances efficiency by restricting memory banks to essential frames. MAVOS \cite{DBLP:journals/corr/abs-2403-17937} optimizes long-term memory usage to ensure temporal smoothness without frequent expansions, and SAM 2 \cite{ravi2024sam2segmentimages} extends memory capabilities with a FIFO queue for seamless object tracking.

\paragraph{Downstream tasks -- action level}
Action classification and localization in videos are critical components of understanding dynamic scenes and require sophisticated models capable of identifying and interpreting temporal patterns. Recent advancements in this field have leveraged memory networks and transformer-based architectures to enhance the accuracy and efficiency of these tasks. One approach that has gained prominence is the use of memory networks. For instance, \cite{DBLP:conf/aaai/00010019} introduces a novel framework that writes significant information into an external memory module while discarding irrelevant data. This selective memory management improves video action recognition by focusing on key temporal elements. Transformer-based models have also been instrumental in advancing action classification and localization. LSTR \cite{DBLP:conf/nips/XuXCLXTS21} utilizes both long-term and short-term memory in a FIFO structure to address online action detection, allowing the model to maintain relevant past information efficiently. MeMViT \cite{DBLP:conf/cvpr/WuLM0XMF22} proposes a hierarchical memory transformer that optimizes long-term memory use for effective video action classification and anticipation. Another significant contribution is RViT \cite{DBLP:conf/cvpr/YangDLZSY22}, which employs an attention gate to facilitate interaction between the current frame input and the previous hidden state. This mechanism enhances the model’s ability to integrate past and present information dynamically. Similarly, MAT \cite{DBLP:conf/iccv/WangCHWL23} introduces a memory encoder that compresses both long-term and short-term memory in a segment-based manner. It also features a memory-anticipation circular decoder that updates historical and future representations for online action detection and anticipation. Finally, MATR \cite{song2024onlinetemporalactionlocalization} presents a FIFO memory queue that selectively retains past segment features, optimizing the process of temporal action localization. This approach ensures that the most relevant temporal features are preserved, improving the model's ability to localize actions accurately over time.


\paragraph{Downstream tasks -- general level}
Video summarization has evolved significantly with the introduction of memory-augmented models and deep learning architectures. Early approaches, such as vsLSTM \cite{DBLP:conf/eccv/ZhangCSG16}, employed LSTM to capture variable-range temporal dependencies among video frames. This method aimed to create both representative and compact video summaries by effectively modeling the temporal relationships inherent in video data. Building on this foundation, MAVS \cite{DBLP:conf/mm/FengLKZ18} introduced a memory-augmented extractive video summarizer that utilized an external memory to store comprehensive visual information from the entire video, enhancing the summarization process with high-capacity memory storage. Furthermore, SMN \cite{DBLP:conf/mm/Wang000FT19} stacked multiple LSTM and memory layers hierarchically. This approach integrated learned representations from prior layers, resulting in more precise video summaries for individual frames by capturing intricate temporal patterns.

Video captioning has also benefited from advancements in memory-augmented networks. M3 \cite{DBLP:conf/cvpr/Wang000T18} proposed attaching an LSTM with an external memory that could store and retrieve both visual and textual content. This method allowed for multiple read and write operations, facilitating rich interactions between video sequences and corresponding sentences. MARN \cite{DBLP:conf/cvpr/PeiZWKST19} introduced the Memory-Attended Recurrent Network, designed to explore the full-spectrum correspondence between words and their visual contexts, enhancing the captioning capabilities by leveraging memory structures. In terms of transformer-based solutions, MART \cite{DBLP:conf/acl/LeiWSYBB20} utilized a layer-wise TransformerXL architecture for video captioning, which was further improved by AAP-MIT \cite{DBLP:journals/tip/PrudvirajRVM22} through the integration of a Pyramid network for generating multi-sentence video descriptions, thereby enriching the narrative depth of the captions.

Video QA tasks have seen significant enhancements through the incorporation of sophisticated memory mechanisms and attention models. The Heterogeneous Memory Enhanced Multimodal Attention Model \cite{DBLP:conf/cvpr/FanZZW0H19} introduced a heterogeneous external memory module on LSTM. This model employed attentional read and write operations to integrate motion and appearance features, co-learning attention mechanisms, and utilizing visual-question interactions to derive global context-aware representations. \cite{DBLP:conf/ijcai/CaiYSLCS20} further advanced Video QA by introducing fine-grained feature-augmented memories. This approach strengthened the information augmentation of video and text, improving memory capacity by capturing global interactions between high-level semantic information through self-attention and co-attention modules. RWMN \cite{DBLP:conf/iccv/NaLKK17} utilized multi-layered CNNs to read and write sequential memory cells as chunks, effectively representing sequential stories with strong inter-block correlations. Lastly, Glance-Focus \cite{DBLP:conf/nips/Bai0023} proposed a two-stage method for Video QA. In the "glance" stage, an Encoder-Decoder generated dynamic event memories without supervision, while in the "focus" stage, these memories bridged the correlation between questions and both high-level event concepts and low-level video content, enhancing the model's comprehension and response accuracy.

\paragraph{Downstream tasks -- others}
In addition to common video understanding tasks, memory-augmented models have been increasingly applied to various other video processing tasks, including flow estimation, depth estimation, video deblurring, gesture recognition, and visual speech recognition. Flow estimation has benefited from models like MemFlow \cite{DBLP:journals/corr/abs-2404-04808}, which employs memory storage for real-time flow estimation, retaining motion information to enhance accuracy. In depth estimation, MAMo \cite{DBLP:conf/iccv/YasarlaCJSGP23} augments networks with memory to store learned visual and displacement tokens from previous frames, allowing for more accurate depth predictions through cross-referencing past features. Video deblurring has advanced with MmDeblur \cite{DBLP:conf/cvpr/JiY22}, which uses a memory branch to memorize blurry-sharp feature pairs, aiding the deblurring process for incoming frames. Gesture recognition has been improved by MENet \cite{DBLP:conf/eccv/SunZCCL22}, which features a dual-branch architecture to capture temporal dynamics between spatiotemporal windows. Visual speech recognition has seen enhancements through frameworks using associative bridges to learn interrelationships and obtain target modal representations from memory \cite{DBLP:conf/iccv/KimHPR21}, with VAM \cite{DBLP:journals/tmm/KimHPR22} imprinting audio features into a memory network using visual features, and MVM \cite{DBLP:conf/aaai/KimYR22} employing multihead key memories for visual features and a value memory for audio knowledge to distinguish homophenes. These applications show the versatility of memory networks in enhancing video understanding systems by leveraging past information for improved accuracy and robustness in complex video analysis scenarios.

\paragraph{Downstream task -- generation}

In the realm of video generation, there is a growing demand for creating long, high-quality videos. This challenge has led to the development of various memory-augmented models that enhance the quality and coherence of generated video content by leveraging advanced memory.

In the realm of video generation, there is a growing demand for creating long, high-quality videos, leading to the development of various memory-augmented models that enhance video content by leveraging advanced memory networks. The LMC-Memory model \cite{DBLP:conf/cvpr/LeeKCKR21} utilizes memory alignment learning to store long-term motion contexts, improving video prediction by matching these contexts with sequences that exhibit limited dynamics. Similarly, MV-TON \cite{DBLP:conf/mm/ZhongWTLW21} introduces a memory refinement module that embeds generated frames into a latent space as external memory, aiding subsequent frame generation with richer context. For talking face video generation, MemGAN \cite{Yi2020AudiodrivenTF} incorporates a memory-augmented GAN module to refine roughly rendered frames into realistic ones, enhancing video quality. Building on this, SyncTalkFace \cite{DBLP:conf/aaai/ParkKHCR22} introduces an Audio-Lip Memory mechanism to align visual information of the mouth region with input audio, ensuring fine-grained audio-visual coherence. The EMMN model \cite{DBLP:conf/iccv/TanJP23} constructs a Motion Memory Net that stores emotion embeddings and mouth motion features as key-value pairs, ensuring consistency between expression and lip motion. STAM \cite{DBLP:journals/tmm/00020WM023} enhances spatiotemporal memorizing capacity by using a SpatioTemporal Attention based Memory on 3D-CNN, incorporating global spatiotemporal information to improve video prediction. Lastly, MemFace \cite{DBLP:journals/corr/abs-2212-05005} addresses missing information in video generation with implicit and explicit memory components, capturing high-level semantics in the audio-expression shared space and aiding the neural-rendering model in synthesizing pixel-level details. These innovations underscore the critical role of memory networks in advancing video generation technology, enabling coherent and visually appealing outputs by effectively integrating past information and context.


% \paragraph{Object Segmentation and Tracking}
% \begin{itemize}
%     % RNN;LSTM;GRU
%     \item ConvGRU\cite{DBLP:conf/iccv/TokmakovAS17} e incorporates a memory unit implemented by convolutional gated recurrent units to capture the evolution of object(s) in the scene 
%     \item RFL\cite{DBLP:conf/iccvw/YangC17} use a convolutional LSTM as the memory unit for video object tracking
%     \item RMAN\cite{DBLP:journals/tip/PuSMZY21} build on top of the long short-term memory network (LSTM) with an additional memory activation layer for visual tracking
%     % memory network
%     \item MemTrack\cite{DBLP:conf/eccv/YangC18} propose a dynamic memory network, where the target information is stored and recalled from external memory, to maintain the variations of object appearance for template-matching, and a LSTM is used to control the reading and writing process of external memory
%     \item STM\cite{DBLP:conf/iccv/OhLXK19} propose a novel DNN system based on the memory network that computes the spatio-temporal attention on every pixel in multiple frames of the video for each pixel in the query image, to decide whether the pixel belongs to a foreground object or not
%     \item STCN\cite{DBLP:conf/nips/ChengTT21} propose using the negative squared Euclidean distance instead to compute the affinities of memory node to improve the efficiency of STM
%     \item STMTrack\cite{DBLP:conf/cvpr/FuLFW21} introduce a memory mechanism stores the historical information of the target to guide the tracker to focus on the most informative regions in the current frame. Furthermore, the pixel-level similarity computation of the memory network enables our tracker to generate much more accurate bounding boxes of the target.
%     \item Motion-Aware Memory Network for Fast Video Salient Object Detection\cite{DBLP:journals/tip/ZhaoLLSZLH24} incoporate the space-time memory-based network to encoder-decoder architecture for video salient object detection
%     \item REMN\cite{DBLP:conf/icmcs/ChenZYW23} t adaptively decide whether to update the memory features depending on the variation of foreground objects to reduce temporal redundancy of memory network for video object segment
%     % Graph network
%     \item GraphMemVOS\cite{DBLP:conf/eccv/LuWDZSG20} exploit an episodic memory network, organized as a fully connected graph, to store frames as nodes and capture cross-frame correlations by edges. Further, learnable controllers are embedded to ease memory reading and writing, as well as maintain a fixed memory scale for video object segmentation
%     \item DTMNet\cite{DBLP:conf/mm/ZhangWLL0L20} propose an  end-to-end network based on graph model which stores short- and long-term video sequence information preceding the current frame as the temporal memories to address the temporal modeling in video object segmentation
%     % other memory
%     \item TMRN\cite{DBLP:conf/iccv/SunWMZW23} are dedicated to improve the memory retrieval operation and we argue that each memory frame should be spatially aligned with the current frame before temporal aggregation for video object segmentation
%     % transformer
%     % tracking
%     % video object segmentation
%     \item AOT\cite{DBLP:conf/nips/YangWY21} propose long-short term memory of past input features and masks, for associaing multiple object segmentation in video.
%     \item IMANet\cite{DBLP:conf/iros/PaulDGT21} aggregates a rich representation of the semantic information in past frames into a memory module. Information stored in the memory is then accessed through an attention mechanism for video semantic segment
%     \item TrackFormer \cite{DBLP:conf/cvpr/MeinhardtKLF22} present recurrent object tracking on transformer to preserve long-term and short-term occlusions
%     \item XMem\cite{DBLP:conf/eccv/ChengS22}following the Atkinson-Shiffrin model, we develop an architecture that incorporates multiple independent yet deeply-connected feature memory stores: a rapidly updated sensory memory, a high-resolution working memory, and a compact thus sustained long-term memory long video object segmentation
%     \item S-ViT\cite{DBLP:conf/cvpr/ZhaoLTCCZ23}; produces frame-level features with a memory-enabled temporally-aware spatial encoder to serve the streaming video  tracking and action classification
%     \item MMC\cite{DBLP:journals/corr/abs-2307-07812} preserve the detailed feature maps during across scale information exchange via a multiscale memory transformer decoding to reduce confusion between the background and novel class on video object segment task.
%     \item RFGM\cite{DBLP:conf/nips/ZhouGHL0GZ23} l tracking paradigm, consisting of a relevance attention mechanism and a global representation memory, which can adaptively assist the search region in selecting the most relevant historical information from reference features.
%     \item RMem\cite{DBLP:journals/corr/abs-2406-08476} restricting memory banks to a limited number of essential frames to improve accuracy and efficiency
%     \item MAVOS\cite{DBLP:journals/corr/abs-2403-17937} introduces an optimized and dynamic long-term modulated cross-attention (MCA) memory to model temporal smoothness without requiring frequent memory expansion for video object segmentation
%     \item  SAM 2\cite{ravi2024sam2segmentimages} extend SAM by FIFO memory queue for tracking object in videos.
% \end{itemize}

% \paragraph{action classification and localization}
% \begin{itemize}
%     % memory network
%     \item Memory-Augmented Temporal Dynamic Learning for Action Recognition\cite{DBLP:conf/aaai/00010019} propose a memory-augmented temporal dynamic learning network, which learns to write the most evident information into an external memory module and ignore irrelevant one for video action recognition
%     % transformer
%     \item LSTR\cite{DBLP:conf/nips/XuXCLXTS21} propose FIFO long term memory and short term memory for online action detection task
%     \item MeMViT\cite{DBLP:conf/cvpr/WuLM0XMF22} propose hierachical (memory) transformer for long term memory for efficient video action classification/anticipation
%     \item RViT\cite{DBLP:conf/cvpr/YangDLZSY22} is equipped with an attention gate to build interaction between current frame input and previous hidden state
%     \item MAT\cite{DBLP:conf/iccv/WangCHWL23} use memory encoder to compress long-term and short-term memory in segment-based fasion, and propose memory-anticipation curcular decoder to perceive the future context and circularly update the historical and future representation for online action detection and anticipation task
%     \item MATR\cite{song2024onlinetemporalactionlocalization} propose FIFO memory queue that selectively preserves the past segment features for temporal action localization
% \end{itemize}




% \paragraph{Video Summarization}
% \begin{itemize}
%     % before transformer
%     \item vsLSTM\cite{DBLP:conf/eccv/ZhangCSG16}  use Long Short-Term Memory (LSTM) to model the variable-range temporal dependency among video frames, so as to derive both representative and compact video summaries
%     \item MAVS\cite{DBLP:conf/mm/FengLKZ18}  proposed a memory augmented extractive video summarizer, which utilizes an external memory to record visual information of the whole video with high capacity.
%     \item SMN\cite{DBLP:conf/mm/Wang000FT19} stack multiple LSTM layers and memory layers hierarchically to integrate the learned representation from prior layers to derive more accurate video summaries for individual video frames
% \end{itemize}


% \paragraph{video caption}
% \begin{itemize}
%     % LSTM;RNN;GRU
%     \item M3\cite{DBLP:conf/cvpr/Wang000T18} propose to attaches LSTM with an external memory to store and retrieve both visual and textual contents by interacting with video and sentence with multiple read and write operations.
%     \item MARN\cite{DBLP:conf/cvpr/PeiZWKST19} propose the Memory-Attended Recurrent Network for video captioning, in which a memory structure is designed to explore the full-spectrum correspondence between a word and its various similar visual contexts across videos in training data.
%     % transformer
%     \item MART\cite{DBLP:conf/acl/LeiWSYBB20} propose layer-wise TransformerXL for video caption
%     \item AAP-MIT\cite{DBLP:journals/tip/PrudvirajRVM22} further improve  MART with Pyramid network for multi-sentence video description
% \end{itemize}

% \paragraph{Video QA}
% \begin{itemize}
%     % rnn;lstm;gru
%     \item Heterogeneous Memory Enhanced Multimodal Attention Model for Video Question Answering\cite{DBLP:conf/cvpr/FanZZW0H19}  introduce a heterogeneous external memory module on LSTM with attentional read and write operations such that the motion and appearance features are integrated to co-learn attention, and utilize the interaction of visual and question features with memory contents to learn global contextaware representations
%     \item Feature Augmented Memory with Global Attention Network for VideoQA\cite{DBLP:conf/ijcai/CaiYSLCS20} introducing two fine-grained feature-augmented memories to strengthen the information augmentation of video and text which can improve the memory capacity by memorizing more relevant and targeted information and appending the self-attention and co-attention module to the memory output thus the module is able to capture global interaction between high-level semantic informations. for videoqa
%     % memory network
%     \item RWMN\cite{DBLP:conf/iccv/NaLKK17}  use of multi-layered CNNs allows the model to read and write sequential memory cells as chunks, which is more reasonable to represent a sequential story because adjacent memory blocks often have strong correlations.
%     % transformer
%     \item Glance-Focus\cite{DBLP:conf/nips/Bai0023} propose a two-stage method for VideoQA, at glance stage,  train an Encoder-Decoder to generate a set of dynamic event memories without supervision, at the focusing stage, these event memories act as a bridge to establish the correlation between the questions with high-level event concepts and low-level lengthy video content

%     % %state space model
%     % \item SHMamba\cite{DBLP:journals/corr/abs-2406-09833} propose  Structured Hyperbolic State Space Model to integrate the advantages of hyperbolic geometry and state space models
% \end{itemize}


% % others

% \paragraph{Flow Estimation}
% \begin{itemize}
%     % flow estimation
%     \item MemFlow \cite{DBLP:journals/corr/abs-2404-04808} store memory for real-time flow estimation
% \end{itemize}

% \paragraph{Depth Estimation}
% \begin{itemize}
%     \item MAMo\cite{DBLP:conf/iccv/YasarlaCJSGP23} augment model with memory which aids the depth prediction as the model streams through the video,  the memory stores learned visual and displacement tokens of the previous time instances. This allows the depth network to cross-reference relevant features from the past when predicting depth on the current frame
% \end{itemize}

% \paragraph{Video Deblurring}
% \begin{itemize}
%     \item MmDeblur\cite{DBLP:conf/cvpr/JiY22}  designed a memory branch based on memory network to memorize the blurry-sharp feature pairs in the memory bank, thus providing useful information for the blurry query input
% \end{itemize}

% \paragraph{Gesture recognition}
% \begin{itemize}
%     \item MENet\cite{DBLP:conf/eccv/SunZCCL22} contains a base branch with a full-sized event point-wise processing structure to extract the base features and an incremental branch equipped with a light-weighted network to capture the temporal dynamics between two adjacent spatiotemporal windows for gesture recognition and object recognition
% \end{itemize}


% \paragraph{visual speech recognition}
% \begin{itemize}
%     % memory network
%     \item \cite{DBLP:conf/iccv/KimHPR21}  learning the interrelationship through the associative bridge, the proposed bridging framework is able to obtain the target modal representations inside the memory network, even with the source modal input only, and it provides rich information for its downstream tasks
%     \item VAM\cite{DBLP:journals/tmm/KimHPR22} propose learns to imprint audio features of short clip-level into a memory network using the corresponding visual features. the model contains two memories, lip-video key and audio value
%     \item MVM\cite{DBLP:conf/aaai/KimYR22}  composed of multihead key memories for saving visual features and one value memory for saving audio knowledge, which is designed to distinguish the homophenes for lip reading
% \end{itemize}

% \paragraph{Video Generation}
% \begin{itemize}
%     % RNN;LSTM;GRU
%     \item LMC-Memory\cite{DBLP:conf/cvpr/LeeKCKR21} memory alignment learning enables to store longterm motion contexts into the memory and to match them with sequences including limited dynamics for video prediction.
%     % memory network
%     \item MV-TON\cite{DBLP:conf/mm/ZhongWTLW21} a memory refinement module that learns to embed the existing generated frames into the latent space as external memory for the following frame generation
%     \item MemGAN\cite{Yi2020AudiodrivenTF} e propose a novel memory-augmented GAN module by incorporated memory to talking face generation to refine roughly rendered frames into realistic frames for talking face video generation
%     \item SyncTalkFace\cite{DBLP:conf/aaai/ParkKHCR22} k proposes Audio-Lip Memory that brings in visual information of the mouth region corresponding to input audio and enforces fine-grained audio-visual coherence for talking face generation
%     \item EMMN\cite{DBLP:conf/iccv/TanJP23} based on memory network construct the Motion Memory Net to store emotion embedding and mouth motion feature and the corresponding expression motion feature as a key-value pair to assure the consistency between expression and lip motion.
%     % other
%     \item STAM\cite{DBLP:journals/tmm/00020WM023} propose a SpatioTemporal Attention based Memory on 3d-CNN, which can efficiently improve the longterm spatiotemporal memorizing capacity by incorporating the global spatiotemporal information in videos for video prediction
%     % transformer
%     \item MemFace\cite{DBLP:journals/corr/abs-2212-05005} propose to e to complement the missing information caused by one-to-many with an implicit memory and an explicit memory that follow the sense of the two stages respectively. More specifically, the implicit memory is employed in the audioto-expression model to capture high-level semantics in the audio-expression shared space, while the explicit memory is employed in the neural-rendering model to help synthesize pixel-level details for talking face generation
% \end{itemize}




\subsubsection{Other Modalities}

Beyond audio and video context modeling, memory strategies are increasingly leveraged across various downstream tasks to enhance context understanding and improve performance. In image captioning, the CSMN model \cite{DBLP:conf/cvpr/ParkKK17} enhances memory networks by using them as repositories for multiple types of context information, appending previously generated words to capture long-term information, and employing a CNN memory structure for better context representation. For anomaly detection, the DAAC model \cite{DBLP:conf/iccv/HouZZXPZ21} modulates reconstruction capabilities by generalizing the memory module in a blockwise manner using a multi-scale approach. In image-to-image translation, MGUIT \cite{DBLP:conf/cvpr/JeongKLS21} explores memory networks to improve translation results. MemoPainter \cite{DBLP:conf/cvpr/YooBCLCC19} introduces a memory-augmented colorization model that achieves high-quality colorization with limited data. For blind face restoration, RMM \cite{DBLP:journals/corr/abs-2110-01033} proposes a wavelet memory module that stores spatial features of low-quality images and guides high-quality restoration. In semantic segmentation, a memory-based approach \cite{DBLP:conf/iros/JinHK21} stores significant training image representations, while MM-Net \cite{DBLP:conf/iccv/WuSL021} uses learnable memory embeddings for few-shot segmentation, and CDFSS \cite{DBLP:conf/cvpr/WangDWEFZ22} employs a meta-memory bank to bridge domain gaps. In deraining, MOSS \cite{DBLP:conf/cvpr/HuangYH21} uses a self-supervised memory module to record prototypical rain patterns. Lastly, for 3D scene reconstruction, TransformerFusion \cite{DBLP:conf/nips/BozicPTDN21} proposes a hierarchical memory of input frame features for online video 3D scene reconstruction. These applications underscore the versatility and effectiveness of memory networks in improving context modeling across diverse tasks.


% \paragraph{Image Caption}
% \begin{itemize}
%     % memory network
%     \item CSMN\cite{DBLP:conf/cvpr/ParkKK17} improve memory network by  exploiting memory as a repository for multiple types of context information, (ii) appending previously generated words into memory to capture long-term information without suffering from the vanishing gradient problem, and (iii) adopting CNN memory structure to jointly represent nearby ordered memory slots for better context understanding for personalized image captioning task.
% \end{itemize}

% \paragraph{anomaly detection}
% \begin{itemize}
%     % memory network
%     \item DAAC\cite{DBLP:conf/iccv/HouZZXPZ21} modulate the reconstruction capability on normality and anomaly by generalizing the memory module to be blockwise rather than pixel-wise in a multi-scale fashion.
    
% \end{itemize}

% \paragraph{Image-to-Image Translation}
% \begin{itemize}
%     % memory network
%     \item MGUIT\cite{DBLP:conf/cvpr/JeongKLS21} explores memory network in Image-to-Image tranlation
% \end{itemize}


% \paragraph{coloralization}
% \begin{itemize}
%     % memory network
%     \item MemoPainter~\cite{DBLP:conf/cvpr/YooBCLCC19} present a novel memory-augmented colorization model that can produce high-quality colorization with limited data on memory network
% \end{itemize}

% \paragraph{blind face restoration}
% \begin{itemize}
%     % memory network
%     \item RMM\cite{DBLP:journals/corr/abs-2110-01033} propose a wavelet memory module that stores spatial features of the low quality images and high-frequency wavelet coefficient information, which enables to adaptively guide the high-quality blind face restoration
% \end{itemize}

% \paragraph{Semantic Segment}
% \begin{itemize}
%     % memory netowrk
%     \item Memory-based Semantic Segmentation for Off-road Unstructured Natural Environments \cite{DBLP:conf/iros/JinHK21} propose memory module stores significant representations of training images as memory items based on memory network for semantic segmentation
%     % memory embedding
%     \item MM-Net\cite{DBLP:conf/iccv/WuSL021} introduce a set of learnable memory embeddings to memorize the meta-class information during the base class training and transfer to novel classes during the inference stage for few-shot semantic segmentation
%     \item CDFSS\cite{DBLP:conf/cvpr/WangDWEFZ22}  meta-memory bank to improve the generalization of the segmentation network by bridging the domain gap between source and target domains. The meta-memory stores the intra-domain style information from source domain instances and transfers it to target samples.
% \end{itemize}

% \paragraph{Deraining}
% \begin{itemize}
%     % memory network
%     \item MOSS\cite{DBLP:conf/cvpr/HuangYH21} designing an encoder-decoder neural network that is augmented with a self-supervised memory module, where items in the memory record the prototypical patterns of rain degradations and are updated in a self-supervised way
% \end{itemize}

% \paragraph{3D Scene Reconstruction}

% \begin{itemize}
%     %  online 3D scene reconstruction 
%     % transformer
%     \item TransformerFusion\cite{DBLP:conf/nips/BozicPTDN21} propose hierachical memory of input frame features for online video 3D scene reconstruction
% \end{itemize}


\subsection{Multimodal Contextual Memory for Vision and Robotics}


Integrating memory mechanisms into the capabilities of embodied agents and robotics has become increasingly essential for enhancing long-term planning, decision-making, visual navigation, and manipulation reasoning. These advancements demonstrate how memory can significantly improve an agent's ability to operate in complex environments.

\subsubsection{Multimodal Memory-Augmented Agents}

Multimodal memory-augmented agents demonstrate the integration of memory in diverse environments. JARVIS-1 \cite{DBLP:journals/corr/abs-2311-05997} equips an agent to perceive multimodal inputs, generate complex plans, and perform embodied control in a gaming environment like Minecraft, using memory to combine pre-trained knowledge with actual game experiences. MM-Navigator \cite{DBLP:journals/corr/abs-2311-07562} employs GPT-4V for multimodal self-summarization in smartphone GUI navigation tasks, converting historical actions into concise natural language memory. MobileGPT \cite{DBLP:journals/corr/abs-2312-03003} and AppAgent \cite{DBLP:journals/corr/abs-2312-13771} focus on smartphone applications, accumulating knowledge about apps in graph form and summarizing interaction histories for improved decision-making and interpretability. OS-Copilot \cite{DBLP:journals/corr/abs-2402-07456} features a framework for building generalist agents capable of interacting with various elements in an operating system, using a configurator with working, declarative, and procedural memory. MEIA \cite{DBLP:journals/corr/abs-2402-00290} offers an embodied agent for cafe scenes, utilizing a multimodal environment memory module that stores key scene information in natural language, guiding large models to execute action plans effectively under diverse requirements.



\subsubsection{Memory-Enhanced Navigation, Odometry, and Manipulation}


\paragraph{Visual Navigation}

In the field of visual navigation, memory mechanisms play a crucial role in enabling agents to navigate effectively. RPF \cite{DBLP:conf/nips/KumarGFLM18} abstracts sequences of images and actions into memories for robust path following using RNNs. SSM \cite{DBLP:conf/cvpr/WangWLXS21} introduces an external structured memory that stores visual and geometric information in disentangled layouts, providing a global action space on LSTM for visual navigation. VGM \cite{DBLP:conf/iccv/KwonKCYPO21} presents visual graph memory based on GCN, which includes unsupervised image representations for navigation history. In the realm of image-goal navigation, memory-augmented reinforcement learning \cite{DBLP:conf/iros/MezghaniSLMBBA22} integrates an external memory mechanism with representations of past observations into the navigation policy. MemoNav \cite{DBLP:journals/corr/abs-2402-19161} introduces a memory model based on GCN and LSTM, attending to short- and long-term memory while efficiently managing memory by forgetting information below a threshold. SMT \cite{DBLP:conf/cvpr/FangT0S19} incorporates attention mechanisms to exploit spatio-temporal dependencies, maintaining long time horizons for navigation. Furthermore, MultiON \cite{DBLP:conf/nips/WaniPJCS20} proposes navigation tasks to test agents' ability to locate previously observed goal objects.

\paragraph{Visual Odometry}

In visual odometry, memory mechanisms also enhance performance. The Deep Visual Odometry With Adaptive Memory model \cite{DBLP:journals/pami/XueWWZ22} employs selective memory based on RNNs to improve visual odometry accuracy and adaptability.

\paragraph{Manipulation Reasoning and Planning}

For manipulation reasoning and planning, RDMemory \cite{DBLP:conf/icra/HuangYKPCLH24} encodes object-oriented memory into a multi-object manipulation framework based on transformers, facilitating sophisticated reasoning and planning capabilities.




% \paragraph{Visual Navigation}

% \begin{itemize}
%     % visual navigation
%     % RNN LSTM GRU
%     \item RPF\cite{DBLP:conf/nips/KumarGFLM18} abstract sequence of images and actions as memoryies for robust path following on RNN.
%     \item SSM\cite{DBLP:conf/cvpr/WangWLXS21} proposed external structured memory, which stores visual and geometric information disentangled layouts and provides global action space for visual navigation on LSTM
%     % graph memory
%     \item VGM\cite{DBLP:conf/iccv/KwonKCYPO21} presents visual graph memory based on GCN, which consist of unsupervised image representations for navigation history for visual navitation
%     \item Memory-Augmented Reinforcement Learning for Image-Goal Navigation\cite{DBLP:conf/iros/MezghaniSLMBBA22}, add an external memory mechanism containing representation of past objservation to the navigation policy for image-goal navigation
%     \item MemoNav\cite{DBLP:journals/corr/abs-2402-19161} present a memory model based on GCN and LSTM, which attented to short/long term memory, forget lower than threshold for efficient visual navigation
%     % transformer
%     \item SMT\cite{DBLP:conf/cvpr/FangT0S19} add each observation to a memory and use the attention mechanism to exploit spatiao-temporal dependencies to keep long time horizons for visual navigation
%     % benchmark
%     \item MultiON\cite{DBLP:conf/nips/WaniPJCS20} prosepo navigation taskss to test the ability of navigation agents  to locate previously observed goal objects.
% \end{itemize}


% \paragraph{Visual Odometry}

% \begin{itemize}
%     % visual odometry
%     % rnn
%     \item Deep Visual Odometry With Adaptive Memory\cite{DBLP:journals/pami/XueWWZ22} presents selective memory based on RNN for visual odometry 
% \end{itemize}


% \paragraph{Manipulation Reasoning and Planning}


% \begin{itemize}
%     % manipulation reasoning and planning 
%     % transformer
%     \item RDMemory\cite{DBLP:conf/icra/HuangYKPCLH24} encode object-oriented memory into a multi-object manipulation reasoning and planning framework based on transformer.    
% \end{itemize}


% \paragraph{Multimodal Memory Augmented Agent}

% \begin{itemize}
%     \item JARVIS-1: Open-World Multi-task Agents with Memory-Augmented Multimodal Language Models\cite{DBLP:journals/corr/abs-2311-05997}, outfit a agent that can perceive multimodal input (visual observations and human instructions), generate sophisticated plans, and perform embodied control on Minescraft with a multimodal memory, which facilitates planning using both pre-trained knowledge and its actual game survival experiences
%     \item MM-Navigator\cite{DBLP:journals/corr/abs-2311-07562} propose agent for smartphone GUI navigation task, at each time step, we ask GPT-4V to perform multimodal self summarization, which converts the historical actions and current step information into a concise history in the form of natural language as memory
%     \item MobileGPT\cite{DBLP:journals/corr/abs-2312-03003} propose agent to propose smartphone designed to accumulate knowledge about the app as a whole, not just the tasks themselves in a format of graph
%     \item AppAgent\cite{DBLP:journals/corr/abs-2312-13771} propose agent to propose smartphone applications, After each action, the agent summarizes the interaction history and the actions taken during the current step. This information is incorporated into the next prompt, which provides the agent with a form of memory. This meticulous approach enhances the reliability and interpretability of the agent’s actions, thereby facilitating more informed decision-making.
%     \item OS-Copilot\cite{DBLP:journals/corr/abs-2402-07456} propose a framework to build generalist agents capable of interfacing with comprehensive elements in an operating system with a configurator consist of working, declarative and procedural memory. the declarative memory store user profile and semantic knowledge, the procedural memory store too repository, the working memory connect previous mentioned two types of memory and planner and actor.
%     \item MEIA\cite{DBLP:journals/corr/abs-2402-00290} propose an embodied agent for cafe scene with multimodal environment memory module, which stores the environment image, the names and coordinates of key items in the scene recorded in natural language as memory, serving as a guidance for the large model to achieve highly executable action plans under diverse needs
    
% \end{itemize}






==> bks/mllm/mllm_memory_rag.tex <==
\subsection{External knowledge/memory augmented MLLM}

In this section, we will introduce MLLM with external knowledge/memory augmentation.

\subsubsection{External Audio/Speech Knowledge/Memory}

\paragraph{Audio Caption}

\begin{itemize}
    \item Audio Captioning using Pre-Trained Large-Scale Language Model Guided by Audio-based Similar Caption Retrieval\cite{DBLP:journals/corr/abs-2012-07331} retrieve audio-text pair for audio caption
    \item RECAP\cite{DBLP:conf/icassp/GhoshKEDM24} retrieve caption for audio caption 
\end{itemize}

\paragraph{ASR}

\begin{itemize}
    \item Using External Off-Policy Speech-To-Text Mappings in Contextual End-To-End Automated Speech Recognition\cite{DBLP:journals/corr/abs-2301-02736} retrieve audio-text embeding by KNN for ASR.
    \item ReSLM\cite{DBLP:conf/icassp/WangSS00YS24}; retrieve text entities mentioned in the audio for ASR
\end{itemize}

\paragraph{Text-To-Audio}
\begin{itemize}
    % retrieval-augmented audio text modeling: speech-to-text/automatic speech to text, audio caption    
    \item Make-An-Audio\cite{DBLP:conf/icml/HuangHY0LLYLYZ23}  retrieve audio-text pair for augment audio generation
    \item Re-AudioLDM\cite{DBLP:conf/icassp/YuanLLHP024} retrieve retrieve text-audio pair for text-to-audio
\end{itemize}


\subsubsection{External Image Knowledge/Memory}

\paragraph{image classification}

\begin{itemize}
    % retrieve image classification
    \item NNCLR\cite{DBLP:conf/iccv/DwibediATSZ21}  samples the nearest neighbors from the dataset in the latent space, and treats them as positives used for contrastive learning to improve image classification
    \item MTN\cite{DBLP:conf/bmvc/IscenBCFS22} use knn-retrieval similar image for class-incremental learning, image classification
    \item Improving Image Recognition by Retrieving from Web-Scale Image-Text Data\cite{DBLP:conf/cvpr/IscenFS23} introduce an attention-based memory module, which learns the importance of each retrieved image example from the memory for image classification
    \item RePrompt\cite{DBLP:journals/corr/abs-2306-02243} present retrieve image-text pair for prompt tuning for image classification
    \item Towards flexible perception with visual memory\cite{geirhos2024flexibleperceptionvisualmemory} construct visual memory by storing image feature from visual encoder, then search neighbors and aggregate the scores for each neighbour with same label, use the highest score to predict the classification label
\end{itemize}

\paragraph{Image Segmentation}
\begin{itemize}
    % retrieve segmentation
    \item kNN-CLIP\cite{DBLP:journals/corr/abs-2404-09447}expand support set by knn for segmentation, training-free 
\end{itemize}


\paragraph{Image Retreieval}

\begin{itemize}
    % retrieve-augmented data for retrieval
    \item KEDs\cite{DBLP:journals/corr/abs-2403-16005} implicitly models the attributes of the reference images by incorporating a database. then retrieve relavant image-caption pair for retrieval
\end{itemize}


\paragraph{Image Caption}

\begin{itemize}
    % rnn;lstm;gru
    \item R2M \cite{DBLP:conf/ijcai/GuoWSW20} implements a concepts-to-sentence memory translator through two-stage memory mechanisms: fusion and recurrent memories, correlating the relational reasoning between common visual concepts and the generated words for long periods
    % other: CNN
    
    % transformer
    % retrieval-augmented image caption
    \item MA-IC\cite{DBLP:conf/aaai/Fei21a} construct a memory bankpre-set matched image-text samples to calibrite the inference probability
    \item RA-Transformer\cite{DBLP:conf/cbmi/SartoCBC22}; retrieve caption by knn for image caption
    \item Smallcap\cite{DBLP:conf/cvpr/Ramos0EK23} propose a lightweight model to retrieve caption for augmentation for image caption  in new domain
    \item AMA\cite{DBLP:conf/bmvc/ChengY23} propose an adaptive memory feedback mechanism to determine the number of k for each target token to prevent retrieved neighbors contain noise in MA-IC
    \item EXTRA\cite{DBLP:conf/eacl/RamosEM23} retrieve caption for augmentation for image caption
    \item PMA-Net\cite{DBLP:conf/iccv/BarracoSCBC23} devise a network which can perform attention over activations obtained while processing other training samples, through a prototypical memory model for image caption
    \item Re-ViLM\cite{DBLP:conf/emnlp/YangPLKNHFYLLS023} built upon the Flamingo, that supports retrieving the relevant knowledge from the external database for zero and in-context few-shot image caption.
    \item EVCap \cite{DBLP:journals/corr/abs-2311-15879}  build ever-changing object knowledge memory using objects’ visuals and names, enabling us to (i) update the memory at a minimal cost and (ii) effortlessly augment LLMs with retrieved object names by utilizing a lightweight and fast-to-train model.
    \item MeaCap\cite{DBLP:journals/corr/abs-2403-03715} equipped with a textual memory, we introduce a retrieve-then-filter module to get key concepts that are highly related to the image for zeroshot image caption
    \item SmallCap\cite{DBLP:conf/acl/LiLRTE24} finds the retrieval-augmented image caption model is sensitive to tokens that appear in the majority of the retrieved captions, and the input attribution shows that those tokens are likely copied into the generated output order retrieval for robustness, therefore they order the caption to improve robustness 
\end{itemize}

\paragraph{VQA}

\begin{itemize}
    % retrieval-augmented vqa
    \item PICa\cite{DBLP:conf/aaai/YangGW0L0W22} convert image to caption then retrieve knowledge for VQA
    \item KAT\cite{DBLP:conf/naacl/GuiWH0BG22} integrates implicit and explicit knowledge in an encoder-decoder architecture to improve performance on OK-VQA
    \item MuRAG\cite{DBLP:conf/emnlp/ChenHCVC22} accesses an external non-parametric multimodal memory to augment language generation. MuRAG is pretrained with a mixture of large-scale imagetext and text-only corpora using a joint contrastive and generative loss
    \item RA-VQA\cite{DBLP:conf/emnlp/LinB22} propose a joint training scheme which includes differentiable  Dense Passage Retrieval (DPR) integrated with answer generation so that the system can be trained in an end-to-end fashion
    \item RASO\cite{DBLP:conf/acl/FuZKPZZLWWCNRX23} adopts PLM to generate all the possible answers, and then trains a lightweight answer selection model for the correct answer. 
    \item FLMR\cite{DBLP:conf/nips/LinCMCB23} incorporates finer-grained, tokenlevel visual and textual features to retrieve knowledge for vqa
    \item ReVeal\cite{DBLP:conf/cvpr/HuI0WCSSRF23} encode external knowledge corpora into key/value pair by V-L Encoder, which could update during training phase. The memory is incoporarted to end-to-end training paradigm for VQA
    \item MPR\cite{DBLP:journals/corr/abs-2306-17675}  integrates retrieved prompts and multimodal features to generate answers
    \item GeReA\cite{DBLP:journals/corr/abs-2402-02503} prompts a MLLM with question relevant vision and language information to generate knowledge-relevant descriptions and use those descriptions for vqa 
\end{itemize}

\paragraph{Visual Dialogue}

\begin{itemize}
    % retrieval-augmnted visual dialogue
    \item KIF\cite{DBLP:journals/tacl/FanGBB21} takes KNN to retrieve multimodal knowledge for dialogue generation
    \item Maria: {A} Visual Experience Powered Conversational Agent\cite{DBLP:conf/acl/LiangHXTGCLJ20} takes text-image retriever aims to retrieve a correlated image to the dialog from an image index, while the visual concept detector extracts rich visual knowledge from the image for visual dialogue generation
    \item VisAD\cite{DBLP:conf/mm/ShenZSSZ21} retrieve image by word (object/object relation/object attribution), which refers as visual impressions for dialogue generation 
\end{itemize}


\paragraph{machine translation}
\begin{itemize}
    % retrieval-augmented machine translation
    \item UVR-NMT\cite{DBLP:conf/iclr/0001C0USLZ20} use a light topic-image lookup table over existing sentence-image pairs to retrieve a group of images with similar topics to the source sentence 
    \item PLUVR\cite{DBLP:conf/acl/FangF22} further retrieve phrase-level image to improve  machine translation
\end{itemize}


\paragraph{visual representation}

\begin{itemize}
    % retrieve image/text for data augmentation 
    %for general model/representation
    
    \item K-LITE\cite{DBLP:conf/nips/ShenL0XYZGWY0KD22} acquired knowledge from WrdNet and Wiktionary is appended to the original textual concepts as model input during pre-training and evaluation to enable zero-shot and few-shot transfer of visual models
    \item LaCLIP\cite{DBLP:conf/nips/FanKIKT23} a simple yet highly effective approach to enhance CLIP training through language rewrites.
    \item RECO\cite{DBLP:conf/iclr/IscenCFS24} propose to equip existing vision-text models with the ability to refine their embedding with cross-modal retrieved information from a memory at inference time, which greatly improves their zero-shot predictions
    \item React\cite{DBLP:conf/cvpr/LiuSY0GLL23} propose framework to acquire the relevant web knowledge to build customized visual models for target domains. They retrieve the most relevant image-text pairs from the web-scale database as external knowledge, and propose to customize the model by only training new modualized blocks while freezing all the original weights
    \item Understanding Retrieval-Augmented Task Adaptation for Vision-Language Models\cite{DBLP:journals/corr/abs-2405-01468} presenting a systematic study to understand the roles of key components in retrieval-augmented adaptation, and highlight the critical role of logit ensemble for effective adaptation, and provide a theoretical results to suppport the empirical observations.
\end{itemize}

\paragraph{Image Enhancement}

\begin{itemize}
    \item EMNet\cite{DBLP:journals/tmm/YeNYWWK24} xternal memory to form an external memory-augmented network  for low-light image enhancement. The external memory aims to capture the sample specific properties of the training dataset to guide the enhancement in the testing phase.
\end{itemize}

\paragraph{Image Generation}

\begin{itemize}
    % retrieval-augmented image generation
    % GAN
    \item RetrieveGAN\cite{DBLP:conf/eccv/TsengLJ0Y20} devise a differentiable retrieval module to retrieve patch for image synthesis on GAN
    \item IC-GAN\cite{DBLP:conf/nips/CasanovaCVDR21} retrieve images near in the latent space of a data point for realistic image generation based on GAN
    % Diffusion
    \item Z-LaVI\cite{DBLP:conf/emnlp/YangYZWYC22}; EMNLP2022; retrieve image then synthesis to inject common knowledge for image generation based on DALLE.
    \item Re-Imagen\cite{DBLP:conf/iclr/ChenHSC23}accesses an external multi-modal knowledge base to retrieve relevant (image, text) pairs and uses them as references to generate the image based on Diffusion
    \item Retrieval-Augmented Diffusion Models\cite{DBLP:conf/nips/BlattmannROMO22}retrieve a set of nearest neighbors from this external database for each training instance and condition the diffusion model and autoregressive model on these informative samples 
    \item kNN-Diffusion\cite{DBLP:conf/iclr/SheyninAPSGNT23} used kNN image embeddings as augmentation for training text-to-image diffusion models without text to solve the lacking of image-text pair problems.
    \item RA-CM3\cite{DBLP:conf/icml/YasunagaAS0LLLZ23} improve CM3 by retrieving image-text pair for image \& text generation
\end{itemize}


\subsubsection{External Video Knowledge/Memory}

\paragraph{Video Caption}

\begin{itemize}
    % retrieval-auagmented data for video captioning
    \item KaVD\cite{DBLP:conf/emnlp/WhiteheadJBCV18} develop an approach that uses video meta-data to retrieve topically related news documents for a video and extracts the events and named entities from these documents for video caption.
    \item MAN\cite{DBLP:journals/tmm/JingZZGSS24} propose visual memory for the encoder to store multiple visual context across videos as external knowledge for video catpion
    \item CM2\cite{DBLP:journals/corr/abs-2404-07610} retrieve text for video caption
    \item Egoinstructor\cite{DBLP:journals/corr/abs-2401-00789} devise a retrieval-augmented multimodal captioning model that automatically retrieves semantically relevant third-person instructional videos to enhance the video captioning of egocentric videos 
\end{itemize}


\paragraph{Video QA}

\begin{itemize}
    % retrieval-augmented video qa
    \item R2A\cite{DBLP:conf/iccvw/PanLGZZWQL23} t retrieves a set of semantically similar texts from a generic text corpus using a pretrained multi-modal model for Video QA task 
\end{itemize}


\paragraph{External 3D Knowledge/Memory}
\begin{itemize}
    % retrieval-augmented 3d generation
    \item ReMoDiffuse\cite{DBLP:conf/iccv/ZhangGPCHLYL23} propose a diffusion-model-based motion generation framework that integrates a retrieval mechanism to refine the denoising process.
    \item AMD\cite{DBLP:conf/aaai/JingZSY024}  (LLM) to parse the input text into a sequence of concise and interpretable anatomical scripts that correspond to the target motion, then use the script to retrieve motion for generating human motion
    \item ReDream\cite{DBLP:journals/corr/abs-2402-02972}  retrieve 3d assets for score distillation sampling-based text-to-3d generation on 2d prior diffusion model
\end{itemize}


\paragraph{Retrieval-Augmented Large language Model}

\begin{itemize}
    % retrieval-agumented llm
    \item RAG-Driver\cite{DBLP:journals/corr/abs-2402-10828}; Arxiv 2402; retrieve video-text pair for MLLM for driving action explanation, justification, and control signal prediction.
    \item Wiki-LLaVA\cite{DBLP:journals/corr/abs-2404-15406}; integrates external knowledge derived from an external memory into the LLaVA model as additional input context
    \item TUNA\cite{DBLP:journals/corr/abs-2406-10839} retrieve tag of images, which contain rich object-aware information such as object names and attributes to improve MLLM
\end{itemize}


\paragraph{Retrieval augmented multimodal agent}
% retrieval augmented agent
\begin{itemize}
    \item AVIS\cite{DBLP:conf/nips/HuI0CSRSF23} combine LLM with external knowledge for VQA
    \item MP5\cite{DBLP:journals/corr/abs-2312-07472} intorduce external knowledge memory for Minecraft task
    \item SearchLVLMs\cite{li2024searchlvlmsplugandplayframeworkaugmenting}combine LVLMs with search engines and website filter
    \item RIR\cite{DBLP:journals/corr/abs-2405-18740} combine LLM with browser-based API for image search, then extract layout explanantion of screenshot to inject LLM with external knowledge.
\end{itemize}










==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/llm_agent/TBD <==
A Survey on the Memory Mechanism of Large Language Model based Agents
===========================
zeyu zhang new wechat survey
===========================
\begin{itemize}
    \item https://github.com/mikekelly/AgentK
    \item memgpt %记忆分级存储，主上下文用于处理当前信息，框架可以根据需要调用和添加外部存储
    \item Context and Time Sensitive Long-term Memory
    \item AriGraph: Learning Knowledge Graph World Models with Episodic Memory for LLM Agents
    \item memagent
    \item metagpt
    \item autogpt
    \item  \url{https://mp.weixin.qq.com/s/SgKruI2_r8NBi7l1zEnvrw}
\end{itemize}
===========================
\textbf{D. Misc}
\begin{itemize}
    \item AIOS %LLM作为OS的一层，听用户需求，调系统指令
    \item supermemory %“Build your own second brain.” 用户可以把喜欢的idea、网页、twitter收藏到这里，调用Mem0来存储，并与其对话，它会在必要时调用以前的记忆查询和调用
\end{itemize}
===========================
Embodied 放在哪？
Open-Ended Instructable Embodied Agents with Memory-Augmented Large Language Models\\
Jarvis-1
===========================
Benchmark就找到这一个，可以忽略?
Evaluating Very Long-Term Conversational Memory of LLM Agents
===========================

% \kyp{System 1 and System 2 do not necessarily correspond to short-term and long-term memory, as both systems can utilize both types of memory. A more fitting analogy would be that System 1 corresponds to shorter chains of thought or directly retrieving usable answers from memory, while System 2 corresponds to longer chains of thought or more formalized reasoning and planning." https://bokcenter.harvard.edu/how-memory-works; https://arxiv.org/pdf/2410.08328; https://arxiv.org/pdf/2309.02427}
===========================

%AS Model Figure
\begin{figure}
    \centering
    \begin{tikzpicture}[node distance=2cm, every node/.style={font=\small}, align=center]
        % Nodes with adjusted text width
        \node (sensory) [draw, rounded corners, fill=red!30, text width=2cm, minimum height=3cm] {Sensory Memory \\ \textit{(The visual information emit from the cell phone.)}};
        \node (shortterm) [draw, rounded corners, fill=blue!30, text width=2cm, minimum height=3cm, right=2.5cm of sensory] {Short-Term Memory \\ \textit{(The target number. Use it in subsequent actions like dialing.)}};
        \node (longterm) [draw, rounded corners, fill=green!30, text width=2cm, minimum height=3cm, right=2.5cm of shortterm] {Long-Term Memory \\ \textit{(This clue for finding the number.)}};
    
        % Arrows between nodes
        \draw[->] (sensory) -- node[midway, above] {Attention} (shortterm);
        \draw[->] (shortterm) -- node[midway, above] {Encoding} (longterm);
        \draw[->, bend left=45] (longterm) to node[text width=3cm, midway, below] {Retrieval \\ \textit{(Recall where to find the number.)}} (shortterm);
    
        % Maintenance rehearsal loop
        \draw[->] (shortterm.east) to[out=60,in=120,looseness=4] node[midway, above] {Maintenance Rehearsal \\ \textit{(Repeating the number to keep in mind.)}} (shortterm.west);
     
        % Input node
        \node (input) [text width=2cm, left=1cm of sensory] {Sensory Input \\ \textit{(A contact list on the cell phone.)}};
        \draw[->] (input) -- (sensory);
    
        % Downward arrows for forgetting with examples
        \draw[->] (sensory.south) -- +(0,-1cm) node[below, text width=2.5cm, align=center] {Forgetting \\ \textit{(Most of the inputs.)}};
        \draw[->] (shortterm.south) -- +(0,-1cm) node[below, text width=2.5cm, align=center] {Forgetting \\ \textit{(The exact number.)}};
        \draw[->] (longterm.south) -- +(0,-1cm) node[below, text width=2.5cm, align=center] {Forgetting \\ \textit{(This clue.)}};
    \end{tikzpicture}
    \caption{The Atkinson-Shiffrin model characterizes memory in terms of stages based on the duration information remains accessible.}
    \label{fig: Atkinson-Shiffrin}
\end{figure}

==> sections/mllm/mllm_memory_rag.tex <==
\subsection{External knowledge/memory augmented MLLM}

In this section, we will introduce MLLM with external knowledge/memory augmentation.

\subsubsection{External Audio/Speech Knowledge/Memory}

\paragraph{Audio Caption}

\begin{itemize}
    \item Audio Captioning using Pre-Trained Large-Scale Language Model Guided by Audio-based Similar Caption Retrieval\cite{DBLP:journals/corr/abs-2012-07331} retrieve audio-text pair for audio caption
    \item RECAP\cite{DBLP:conf/icassp/GhoshKEDM24} retrieve caption for audio caption 
\end{itemize}

\paragraph{ASR}

\begin{itemize}
    \item Using External Off-Policy Speech-To-Text Mappings in Contextual End-To-End Automated Speech Recognition\cite{DBLP:journals/corr/abs-2301-02736} retrieve audio-text embeding by KNN for ASR.
    \item ReSLM\cite{DBLP:conf/icassp/WangSS00YS24}; retrieve text entities mentioned in the audio for ASR
\end{itemize}

\paragraph{Text-To-Audio}
\begin{itemize}
    % retrieval-augmented audio text modeling: speech-to-text/automatic speech to text, audio caption    
    \item Make-An-Audio\cite{DBLP:conf/icml/HuangHY0LLYLYZ23}  retrieve audio-text pair for augment audio generation
    \item Re-AudioLDM\cite{DBLP:conf/icassp/YuanLLHP024} retrieve retrieve text-audio pair for text-to-audio
\end{itemize}


\subsubsection{External Image Knowledge/Memory}

\paragraph{image classification}

\begin{itemize}
    % retrieve image classification
    \item NNCLR\cite{DBLP:conf/iccv/DwibediATSZ21}  samples the nearest neighbors from the dataset in the latent space, and treats them as positives used for contrastive learning to improve image classification
    \item MTN\cite{DBLP:conf/bmvc/IscenBCFS22} use knn-retrieval similar image for class-incremental learning, image classification
    \item Improving Image Recognition by Retrieving from Web-Scale Image-Text Data\cite{DBLP:conf/cvpr/IscenFS23} introduce an attention-based memory module, which learns the importance of each retrieved image example from the memory for image classification
    \item RePrompt\cite{DBLP:journals/corr/abs-2306-02243} present retrieve image-text pair for prompt tuning for image classification
    \item Towards flexible perception with visual memory\cite{geirhos2024flexibleperceptionvisualmemory} construct visual memory by storing image feature from visual encoder, then search neighbors and aggregate the scores for each neighbour with same label, use the highest score to predict the classification label
\end{itemize}

\paragraph{Image Segmentation}
\begin{itemize}
    % retrieve segmentation
    \item kNN-CLIP\cite{DBLP:journals/corr/abs-2404-09447}expand support set by knn for segmentation, training-free 
\end{itemize}


\paragraph{Image Retreieval}

\begin{itemize}
    % retrieve-augmented data for retrieval
    \item KEDs\cite{DBLP:journals/corr/abs-2403-16005} implicitly models the attributes of the reference images by incorporating a database. then retrieve relavant image-caption pair for retrieval
\end{itemize}


\paragraph{Image Caption}

\begin{itemize}
    % rnn;lstm;gru
    \item R2M \cite{DBLP:conf/ijcai/GuoWSW20} implements a concepts-to-sentence memory translator through two-stage memory mechanisms: fusion and recurrent memories, correlating the relational reasoning between common visual concepts and the generated words for long periods
    % other: CNN
    
    % transformer
    % retrieval-augmented image caption
    \item MA-IC\cite{DBLP:conf/aaai/Fei21a} construct a memory bankpre-set matched image-text samples to calibrite the inference probability
    \item RA-Transformer\cite{DBLP:conf/cbmi/SartoCBC22}; retrieve caption by knn for image caption
    \item Smallcap\cite{DBLP:conf/cvpr/Ramos0EK23} propose a lightweight model to retrieve caption for augmentation for image caption  in new domain
    \item AMA\cite{DBLP:conf/bmvc/ChengY23} propose an adaptive memory feedback mechanism to determine the number of k for each target token to prevent retrieved neighbors contain noise in MA-IC
    \item EXTRA\cite{DBLP:conf/eacl/RamosEM23} retrieve caption for augmentation for image caption
    \item PMA-Net\cite{DBLP:conf/iccv/BarracoSCBC23} devise a network which can perform attention over activations obtained while processing other training samples, through a prototypical memory model for image caption
    \item Re-ViLM\cite{DBLP:conf/emnlp/YangPLKNHFYLLS023} built upon the Flamingo, that supports retrieving the relevant knowledge from the external database for zero and in-context few-shot image caption.
    \item EVCap \cite{DBLP:journals/corr/abs-2311-15879}  build ever-changing object knowledge memory using objects’ visuals and names, enabling us to (i) update the memory at a minimal cost and (ii) effortlessly augment LLMs with retrieved object names by utilizing a lightweight and fast-to-train model.
    \item MeaCap\cite{DBLP:journals/corr/abs-2403-03715} equipped with a textual memory, we introduce a retrieve-then-filter module to get key concepts that are highly related to the image for zeroshot image caption
    \item SmallCap\cite{DBLP:conf/acl/LiLRTE24} finds the retrieval-augmented image caption model is sensitive to tokens that appear in the majority of the retrieved captions, and the input attribution shows that those tokens are likely copied into the generated output order retrieval for robustness, therefore they order the caption to improve robustness 
\end{itemize}

\paragraph{VQA}

\begin{itemize}
    % retrieval-augmented vqa
    \item PICa\cite{DBLP:conf/aaai/YangGW0L0W22} convert image to caption then retrieve knowledge for VQA
    \item KAT\cite{DBLP:conf/naacl/GuiWH0BG22} integrates implicit and explicit knowledge in an encoder-decoder architecture to improve performance on OK-VQA
    \item MuRAG\cite{DBLP:conf/emnlp/ChenHCVC22} accesses an external non-parametric multimodal memory to augment language generation. MuRAG is pretrained with a mixture of large-scale imagetext and text-only corpora using a joint contrastive and generative loss
    \item RA-VQA\cite{DBLP:conf/emnlp/LinB22} propose a joint training scheme which includes differentiable  Dense Passage Retrieval (DPR) integrated with answer generation so that the system can be trained in an end-to-end fashion
    \item RASO\cite{DBLP:conf/acl/FuZKPZZLWWCNRX23} adopts PLM to generate all the possible answers, and then trains a lightweight answer selection model for the correct answer. 
    \item FLMR\cite{DBLP:conf/nips/LinCMCB23} incorporates finer-grained, tokenlevel visual and textual features to retrieve knowledge for vqa
    \item ReVeal\cite{DBLP:conf/cvpr/HuI0WCSSRF23} encode external knowledge corpora into key/value pair by V-L Encoder, which could update during training phase. The memory is incoporarted to end-to-end training paradigm for VQA
    \item MPR\cite{DBLP:journals/corr/abs-2306-17675}  integrates retrieved prompts and multimodal features to generate answers
    \item GeReA\cite{DBLP:journals/corr/abs-2402-02503} prompts a MLLM with question relevant vision and language information to generate knowledge-relevant descriptions and use those descriptions for vqa 
\end{itemize}

\paragraph{Visual Dialogue}

\begin{itemize}
    % retrieval-augmnted visual dialogue
    \item KIF\cite{DBLP:journals/tacl/FanGBB21} takes KNN to retrieve multimodal knowledge for dialogue generation
    \item Maria: {A} Visual Experience Powered Conversational Agent\cite{DBLP:conf/acl/LiangHXTGCLJ20} takes text-image retriever aims to retrieve a correlated image to the dialog from an image index, while the visual concept detector extracts rich visual knowledge from the image for visual dialogue generation
    \item VisAD\cite{DBLP:conf/mm/ShenZSSZ21} retrieve image by word (object/object relation/object attribution), which refers as visual impressions for dialogue generation 
\end{itemize}


\paragraph{machine translation}
\begin{itemize}
    % retrieval-augmented machine translation
    \item UVR-NMT\cite{DBLP:conf/iclr/0001C0USLZ20} use a light topic-image lookup table over existing sentence-image pairs to retrieve a group of images with similar topics to the source sentence 
    \item PLUVR\cite{DBLP:conf/acl/FangF22} further retrieve phrase-level image to improve  machine translation
\end{itemize}


\paragraph{visual representation}

\begin{itemize}
    % retrieve image/text for data augmentation 
    %for general model/representation
    
    \item K-LITE\cite{DBLP:conf/nips/ShenL0XYZGWY0KD22} acquired knowledge from WrdNet and Wiktionary is appended to the original textual concepts as model input during pre-training and evaluation to enable zero-shot and few-shot transfer of visual models
    \item LaCLIP\cite{DBLP:conf/nips/FanKIKT23} a simple yet highly effective approach to enhance CLIP training through language rewrites.
    \item RECO\cite{DBLP:conf/iclr/IscenCFS24} propose to equip existing vision-text models with the ability to refine their embedding with cross-modal retrieved information from a memory at inference time, which greatly improves their zero-shot predictions
    \item React\cite{DBLP:conf/cvpr/LiuSY0GLL23} propose framework to acquire the relevant web knowledge to build customized visual models for target domains. They retrieve the most relevant image-text pairs from the web-scale database as external knowledge, and propose to customize the model by only training new modualized blocks while freezing all the original weights
    \item Understanding Retrieval-Augmented Task Adaptation for Vision-Language Models\cite{DBLP:journals/corr/abs-2405-01468} presenting a systematic study to understand the roles of key components in retrieval-augmented adaptation, and highlight the critical role of logit ensemble for effective adaptation, and provide a theoretical results to suppport the empirical observations.
\end{itemize}

\paragraph{Image Enhancement}

\begin{itemize}
    \item EMNet\cite{DBLP:journals/tmm/YeNYWWK24} xternal memory to form an external memory-augmented network  for low-light image enhancement. The external memory aims to capture the sample specific properties of the training dataset to guide the enhancement in the testing phase.
\end{itemize}

\paragraph{Image Generation}

\begin{itemize}
    % retrieval-augmented image generation
    % GAN
    \item RetrieveGAN\cite{DBLP:conf/eccv/TsengLJ0Y20} devise a differentiable retrieval module to retrieve patch for image synthesis on GAN
    \item IC-GAN\cite{DBLP:conf/nips/CasanovaCVDR21} retrieve images near in the latent space of a data point for realistic image generation based on GAN
    % Diffusion
    \item Z-LaVI\cite{DBLP:conf/emnlp/YangYZWYC22}; EMNLP2022; retrieve image then synthesis to inject common knowledge for image generation based on DALLE.
    \item Re-Imagen\cite{DBLP:conf/iclr/ChenHSC23}accesses an external multi-modal knowledge base to retrieve relevant (image, text) pairs and uses them as references to generate the image based on Diffusion
    \item Retrieval-Augmented Diffusion Models\cite{DBLP:conf/nips/BlattmannROMO22}retrieve a set of nearest neighbors from this external database for each training instance and condition the diffusion model and autoregressive model on these informative samples 
    \item kNN-Diffusion\cite{DBLP:conf/iclr/SheyninAPSGNT23} used kNN image embeddings as augmentation for training text-to-image diffusion models without text to solve the lacking of image-text pair problems.
    \item RA-CM3\cite{DBLP:conf/icml/YasunagaAS0LLLZ23} improve CM3 by retrieving image-text pair for image \& text generation
\end{itemize}


\subsubsection{External Video Knowledge/Memory}

\paragraph{Video Caption}

\begin{itemize}
    % retrieval-auagmented data for video captioning
    \item KaVD\cite{DBLP:conf/emnlp/WhiteheadJBCV18} develop an approach that uses video meta-data to retrieve topically related news documents for a video and extracts the events and named entities from these documents for video caption.
    \item MAN\cite{DBLP:journals/tmm/JingZZGSS24} propose visual memory for the encoder to store multiple visual context across videos as external knowledge for video catpion
    \item CM2\cite{DBLP:journals/corr/abs-2404-07610} retrieve text for video caption
    \item Egoinstructor\cite{DBLP:journals/corr/abs-2401-00789} devise a retrieval-augmented multimodal captioning model that automatically retrieves semantically relevant third-person instructional videos to enhance the video captioning of egocentric videos 
\end{itemize}


\paragraph{Video QA}

\begin{itemize}
    % retrieval-augmented video qa
    \item R2A\cite{DBLP:conf/iccvw/PanLGZZWQL23} t retrieves a set of semantically similar texts from a generic text corpus using a pretrained multi-modal model for Video QA task 
\end{itemize}


\paragraph{External 3D Knowledge/Memory}
\begin{itemize}
    % retrieval-augmented 3d generation
    \item ReMoDiffuse\cite{DBLP:conf/iccv/ZhangGPCHLYL23} propose a diffusion-model-based motion generation framework that integrates a retrieval mechanism to refine the denoising process.
    \item AMD\cite{DBLP:conf/aaai/JingZSY024}  (LLM) to parse the input text into a sequence of concise and interpretable anatomical scripts that correspond to the target motion, then use the script to retrieve motion for generating human motion
    \item ReDream\cite{DBLP:journals/corr/abs-2402-02972}  retrieve 3d assets for score distillation sampling-based text-to-3d generation on 2d prior diffusion model
\end{itemize}


\paragraph{Retrieval-Augmented Large language Model}

\begin{itemize}
    % retrieval-agumented llm
    \item RAG-Driver\cite{DBLP:journals/corr/abs-2402-10828}; Arxiv 2402; retrieve video-text pair for MLLM for driving action explanation, justification, and control signal prediction.
    \item Wiki-LLaVA\cite{DBLP:journals/corr/abs-2404-15406}; integrates external knowledge derived from an external memory into the LLaVA model as additional input context
    \item TUNA\cite{DBLP:journals/corr/abs-2406-10839} retrieve tag of images, which contain rich object-aware information such as object names and attributes to improve MLLM
\end{itemize}


\paragraph{Retrieval augmented multimodal agent}
% retrieval augmented agent
\begin{itemize}
    \item AVIS\cite{DBLP:conf/nips/HuI0CSRSF23} combine LLM with external knowledge for VQA
    \item MP5\cite{DBLP:journals/corr/abs-2312-07472} intorduce external knowledge memory for Minecraft task
    \item SearchLVLMs\cite{li2024searchlvlmsplugandplayframeworkaugmenting}combine LVLMs with search engines and website filter
    \item RIR\cite{DBLP:journals/corr/abs-2405-18740} combine LLM with browser-based API for image search, then extract layout explanantion of screenshot to inject LLM with external knowledge.
\end{itemize}










==> sections/mllm/mllm_taxonomy.tex <==
\definecolor{ml}{HTML}{d3e6f1}
\definecolor{ml_lr}{HTML}{e8daee}
\definecolor{ml_lr2}{HTML}{ebdef0}
\definecolor{ml_lr2_text}{HTML}{f4ebf7}
\definecolor{ml_la}{HTML}{d6eaf8}
\definecolor{ml_la2}{HTML}{ebf5fb}
\definecolor{ml_la2_text}{HTML}{fef9e7}

\definecolor{mr}{HTML}{fadbd8}
\definecolor{mr2}{HTML}{fdedeb}
\definecolor{mr_text}{HTML}{fdedeb}

\definecolor{myred}{HTML}{f5b6b1}

% \begin{figure}[!htbp]
% \centering
% \tikzset{
%     basic/.style  = {draw, text width=2cm, align=center, font=\sffamily, rectangle},
%     root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=white,text width=8cm, rotate=90, font=\footnotesize},
%     dnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
%     dnode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize},
%     mnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=myred, draw=myred, text width=2.2cm, font=\footnotesize},
%     mnode_p/.style = {basic, thin, rounded corners=2pt, align=center, fill=mr,draw=mr, text width=2.2cm, font=\footnotesize},
%     mnode_p2/.style = {basic, thin, rounded corners=2pt, align=center, fill=mr2, draw=mr2, text width=2cm, font=\footnotesize},
%     mnode_l/.style = {basic, thin, rounded corners=2pt, align=center, fill=ml, draw=ml, text width=2.2cm, font=\footnotesize},
%     mnode_la/.style = {basic, thin, rounded corners=2pt, align=center, fill=ml_la, draw=ml_la, text width=2cm, font=\footnotesize},
%     mnode_la2/.style = {basic, thin, rounded corners=2pt, align=center, fill=ml_la2, draw=ml_la2, text width=2cm, font=\footnotesize},
%     mnode_lr/.style = {basic, thin, rounded corners=2pt, align=center, fill=ml_lr, draw=ml_lr, text width=2cm, font=\footnotesize},
%     mnode_lr2/.style = {basic, thin, rounded corners=2pt, align=center, fill=ml_lr2, draw=ml_lr2, text width=2cm, font=\footnotesize},
%     mnode_2/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
%     mnode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize}, 
%     snode/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2.5cm, font=\footnotesize},
%     snode_1/.style = {basic, thin, rounded corners=2pt, align=center, fill=beaublue!40,text width=2cm, font=\footnotesize},
%     tnode/.style = {basic, thin, align=left, fill=pink!60, text width=15em, align=center},
%     xnode/.style = {basic, thin, rounded corners=2pt, align=center, fill=blue!20,text width=5cm,},
%     wnode_mr/.style = {basic, thick, rounded corners=2pt, align=left, fill=white, draw=mr, text width=5.15cm, font=\footnotesize},
%     wnode_1/.style = {basic, thick, rounded corners=2pt, align=left, fill=white, draw=ml_la, text width=2.5cm, font=\footnotesize},
%     wnode_2/.style = {basic, thick, rounded corners=2pt, align=left, fill=white, draw=ml_lr, text width=2.5cm, font=\footnotesize},
% }
% %
% \begin{forest} 
% for tree={
%     grow=east,
%     growth parent anchor=east,
%     parent anchor=east,
%     child anchor=west,
%     edge path={\noexpand\path[\forestoption{edge},->, >={latex}] 
%          (!u.parent anchor) -- +(5pt,0pt) |- (.child anchor)
%          \forestoption{edge label};}
% }
% % c sep is used for arrow distance
% [Memory-augmented MLLM, mnode    
%     [Multimodal Context Modeling with Memory, mnode_l 
%         [Audio Context Modeling , mnode_la
%             [
%             {
%             Conformer-NTM \citep{DBLP:conf/interspeech/CarvalhoA23},
%             Loop-Copilot \citep{DBLP:journals/corr/abs-2310-12404},
%             MR-MT3 \citep{DBLP:journals/corr/abs-2403-10024}
%             }, wnode_1
%             ]
%         ]
%         [Video Context Modeling, mnode_lr
%             [
%             Video Representation Learning, mnode_lr2
%                 [
%                 {
%                 MC-ViT \citep{DBLP:journals/corr/abs-2402-05861}
%                 }, wnode_1
%                 ]
%             ]
%             [
%             Large Video Language Models, mnode_lr2
%                 [
%                 {
%                 MovieChat \citep{DBLP:journals/corr/abs-2307-16449},
%                 MA-LMM \citep{DBLP:journals/corr/abs-2404-05726},
%                 VideoStreaming \citep{DBLP:journals/corr/abs-2405-16009},
%                 Flash-VStream \citep{DBLP:journals/corr/abs-2406-08085},
%                 VideoLLaMB\citep{wang2024videollamblongcontextvideounderstanding},
%                 OmniDrive \citep{wang2024omnidriveholisticllmagentframework}
%                 }, wnode_1
%                 ]
%             ]
%             [
%             Video Agent, mnode_lr2
%                 [
%                 {
%                 LLoVi \citep{DBLP:journals/corr/abs-2312-17235},
%                 LifelongMemory \citep{DBLP:journals/corr/abs-2312-05269},
%                 VideoAgent\citep{DBLP:journals/corr/abs-2403-10517},
%                 VideoAgent \citep{DBLP:journals/corr/abs-2403-11481},
%                 ChatVideo \citep{DBLP:journals/corr/abs-2304-14407},
%                 DoraemonGPT \citep{DBLP:journals/corr/abs-2401-08392},
%                 LangRepo \citep{DBLP:journals/corr/abs-2403-14622},
%                 DrVideo \citep{DBLP:journals/corr/abs-2406-12846}
%                 }, wnode_1
%                 ]
%             ]
%         ]
%         [Other Modalities, mnode_lr
%             [
%             {
%             CSMN model \citep{DBLP:conf/cvpr/ParkKK17},
%             DAAC model \citep{DBLP:conf/iccv/HouZZXPZ21},
%             MGUIT \citep{DBLP:conf/cvpr/JeongKLS21},
%             MemoPainter \citep{DBLP:conf/cvpr/YooBCLCC19},
%             RMM \citep{DBLP:journals/corr/abs-2110-01033},
%             \citep{DBLP:conf/iros/JinHK21},
%             MM-Net \citep{DBLP:conf/iccv/WuSL021},
%             CDFSS \citep{DBLP:conf/cvpr/WangDWEFZ22},
%             MOSS \citep{DBLP:conf/cvpr/HuangYH21},
%             TransformerFusion \citep{DBLP:conf/nips/BozicPTDN21}
%             }, wnode_1
%             ]
%         ]
%     ]
%     [Multimodal Contextual Memory for Vision and Robotics , mnode_p,
%         [Multimodal Memory-Augmented Agents, mnode_p2
%             [
%             {
%             JARVIS-1 \citep{DBLP:journals/corr/abs-2311-05997},
%             MM-Navigator \citep{DBLP:journals/corr/abs-2311-07562},
%             MobileGPT \citep{DBLP:journals/corr/abs-2312-03003},
%             AppAgent \citep{DBLP:journals/corr/abs-2312-13771},
%             OS-Copilot \citep{DBLP:journals/corr/abs-2402-07456},
%             MEIA \citep{DBLP:journals/corr/abs-2402-00290}
%             }, wnode_1
%             ]
%         ]
%         [{Memory-Enhanced Navigation, Odometry, and Manipulation}, mnode_p2
%            [
%            Visual Navigation, mnode_lr2
%                 [
%                 {
%                 RPF \citep{DBLP:conf/nips/KumarGFLM18},
%                 SSM \citep{DBLP:conf/cvpr/WangWLXS21},
%                 VGM \citep{DBLP:conf/iccv/KwonKCYPO21},
%                 \citep{DBLP:conf/iros/MezghaniSLMBBA22},
%                 MemoNav \citep{DBLP:journals/corr/abs-2402-19161},
%                 SMT \citep{DBLP:conf/cvpr/FangT0S19},
%                 MultiON \citep{DBLP:conf/nips/WaniPJCS20}
%                 }, wnode_1
%                 ]
%            ]
%            [
%            Visual Odometry, mnode_lr2
%                 [
%                 {
%                 Deep Visual Odometry With Adaptive Memory model \citep{DBLP:journals/pami/XueWWZ22}
%                 }, wnode_1
%                 ]
%            ]
%            [
%            Manipulation Reasoning and Planning, mnode_lr2
%                 [
%                 {
%                 RDMemory \citep{DBLP:conf/icra/HuangYKPCLH24}
%                 }, wnode_1
%                 ]
%            ]
%         ]
%     ]
% ]
% \end{forest}
% \caption{Taxonomy of Memory-augmented Multi-Modal Large Language models}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\newcommand{\firstcolumnwidth}{2cm}
\newcommand{\secondcolumnwidth}{2cm}
\newcommand{\audiocontextmodeling}{\makecell[l]{Conformer-NTM \citep{DBLP:conf/interspeech/CarvalhoA23},\\
            Loop-Copilot \citep{DBLP:journals/corr/abs-2310-12404},\\
            MR-MT3 \citep{DBLP:journals/corr/abs-2403-10024}}
            }
\newcommand{\videoreprlearning}{\makecell[l]{MC-ViT \citep{DBLP:journals/corr/abs-2402-05861}}}
\newcommand{\lvlm}{\makecell[l]{MovieChat \citep{DBLP:journals/corr/abs-2307-16449},\\
                MA-LMM \citep{DBLP:journals/corr/abs-2404-05726},\\
                VideoStreaming \citep{DBLP:journals/corr/abs-2405-16009},\\
                Flash-VStream \citep{DBLP:journals/corr/abs-2406-08085},\\
                VideoLLaMB\citep{wang2024videollamblongcontextvideounderstanding},\\
                OmniDrive \citep{wang2024omnidriveholisticllmagentframework}}}
\newcommand{\videoagent}{\makecell[l]{LLoVi \citep{DBLP:journals/corr/abs-2312-17235},\\
                LifelongMemory \citep{DBLP:journals/corr/abs-2312-05269},\\
                VideoAgent\citep{DBLP:journals/corr/abs-2403-10517},\\
                VideoAgent \citep{DBLP:journals/corr/abs-2403-11481},\\
                ChatVideo \citep{DBLP:journals/corr/abs-2304-14407},\\
                DoraemonGPT \citep{DBLP:journals/corr/abs-2401-08392},\\
                LangRepo \citep{DBLP:journals/corr/abs-2403-14622},\\
                DrVideo \citep{DBLP:journals/corr/abs-2406-12846}}}
\newcommand{\othermodalities}{\makecell[l]{CSMN model \citep{DBLP:conf/cvpr/ParkKK17},
            DAAC model \citep{DBLP:conf/iccv/HouZZXPZ21},\\
            MGUIT \citep{DBLP:conf/cvpr/JeongKLS21},
            MemoPainter \citep{DBLP:conf/cvpr/YooBCLCC19},\\
            RMM \citep{DBLP:journals/corr/abs-2110-01033},
            \citep{DBLP:conf/iros/JinHK21},\\
            MM-Net \citep{DBLP:conf/iccv/WuSL021},
            CDFSS \citep{DBLP:conf/cvpr/WangDWEFZ22},\\
            MOSS \citep{DBLP:conf/cvpr/HuangYH21},
            TransformerFusion \citep{DBLP:conf/nips/BozicPTDN21}}}
\newcommand{\object}{\makecell[l]{ConvGRU \citep{DBLP:conf/iccv/TokmakovAS17},
RFL \citep{DBLP:conf/iccvw/YangC17},\\
RMAN \citep{DBLP:journals/tip/PuSMZY21},
MemTrack \citep{DBLP:conf/eccv/YangC18},\\
STM \citep{DBLP:conf/iccv/OhLXK19},
STCN \citep{DBLP:conf/nips/ChengTT21},\\
STMTrack \citep{DBLP:conf/cvpr/FuLFW21},
GraphMemVOS \citep{DBLP:conf/eccv/LuWDZSG20},\\
DTMNet \citep{DBLP:conf/mm/ZhangWLL0L20},
TMRN \citep{DBLP:conf/iccv/SunWMZW23},\\
AOT \citep{DBLP:conf/nips/YangWY21},
IMANet \citep{DBLP:conf/iros/PaulDGT21},\\
TrackFormer \citep{DBLP:conf/cvpr/MeinhardtKLF22},
XMem \citep{DBLP:conf/eccv/ChengS22},\\
S-ViT \citep{DBLP:conf/cvpr/ZhaoLTCCZ23},
MMC \citep{DBLP:journals/corr/abs-2307-07812},\\
RFGM \citep{DBLP:conf/nips/ZhouGHL0GZ23},
RMem \citep{DBLP:journals/corr/abs-2406-08476},\\
MAVOS \citep{DBLP:journals/corr/abs-2403-17937},
SAM 2 \citep{ravi2024sam2segmentimages}.}}
\newcommand{\action}{\makecell[l]{\citep{DBLP:conf/aaai/00010019},
LSTR \citep{DBLP:conf/nips/XuXCLXTS21},\\
MeMViT \citep{DBLP:conf/cvpr/WuLM0XMF22},
RViT \citep{DBLP:conf/cvpr/YangDLZSY22},\\
MAT \citep{DBLP:conf/iccv/WangCHWL23},
MATR \citep{song2024onlinetemporalactionlocalization}.}}
\newcommand{\general}{\makecell[l]{vsLSTM \citep{DBLP:conf/eccv/ZhangCSG16},
MAVS \citep{DBLP:conf/mm/FengLKZ18},\\
SMN \citep{DBLP:conf/mm/Wang000FT19},
M3 \citep{DBLP:conf/cvpr/Wang000T18},\\
MARN \citep{DBLP:conf/cvpr/PeiZWKST19},
MART \citep{DBLP:conf/acl/LeiWSYBB20},\\
AAP-MIT \citep{DBLP:journals/tip/PrudvirajRVM22},\\
Heterogeneous Memory Enhanced Multimodal Attention Model \citep{DBLP:conf/cvpr/FanZZW0H19},\\
\citep{DBLP:conf/ijcai/CaiYSLCS20},
RWMN \citep{DBLP:conf/iccv/NaLKK17},
Glance-Focus \citep{DBLP:conf/nips/Bai0023}.}}
\newcommand{\others}{\makecell[l]{MemFlow \citep{DBLP:journals/corr/abs-2404-04808},
MAMo \citep{DBLP:conf/iccv/YasarlaCJSGP23},\\
MmDeblur \citep{DBLP:conf/cvpr/JiY22},
MENet \citep{DBLP:conf/eccv/SunZCCL22},\\
\citep{DBLP:conf/iccv/KimHPR21},
VAM \citep{DBLP:journals/tmm/KimHPR22},\\
MVM \citep{DBLP:conf/aaai/KimYR22}.}}
\newcommand{\generation}{\makecell[l]{LMC-Memory \citep{DBLP:conf/cvpr/LeeKCKR21},
MV-TON \citep{DBLP:conf/mm/ZhongWTLW21},\\
MemGAN \citep{Yi2020AudiodrivenTF},
SyncTalkFace \citep{DBLP:conf/aaai/ParkKHCR22},\\
EMMN \citep{DBLP:conf/iccv/TanJP23},
STAM \citep{DBLP:journals/tmm/00020WM023},\\
MemFace \citep{DBLP:journals/corr/abs-2212-05005}.}}
\newcommand{\mmmemoryaugmentedagent}{\makecell[l]{JARVIS-1 \citep{DBLP:journals/corr/abs-2311-05997},
            MM-Navigator \citep{DBLP:journals/corr/abs-2311-07562},\\
            MobileGPT \citep{DBLP:journals/corr/abs-2312-03003},
            AppAgent \citep{DBLP:journals/corr/abs-2312-13771},\\
            OS-Copilot \citep{DBLP:journals/corr/abs-2402-07456},
            MEIA \citep{DBLP:journals/corr/abs-2402-00290}}}
\newcommand{\navigation}{\makecell[l]{RPF \citep{DBLP:conf/nips/KumarGFLM18},\\
                SSM \citep{DBLP:conf/cvpr/WangWLXS21},\\
                VGM \citep{DBLP:conf/iccv/KwonKCYPO21},\\
                \citep{DBLP:conf/iros/MezghaniSLMBBA22},\\
                MemoNav \citep{DBLP:journals/corr/abs-2402-19161},\\
                SMT \citep{DBLP:conf/cvpr/FangT0S19},\\
                MultiON \citep{DBLP:conf/nips/WaniPJCS20}}}
\newcommand{\odometry}{\makecell[l]{Deep Visual Odometry\\ With Adaptive Memory model\\ \citep{DBLP:journals/pami/XueWWZ22}}}
\newcommand{\manipulation}{\makecell[l]{RDMemory \citep{DBLP:conf/icra/HuangYKPCLH24}}}

\begin{table}[!htbp]\scriptsize
% \renewcommand\arraystretch{2}
% \resizebox{\textwidth}{4cm}{
% \begin{tabular}{|c|>{\centering\arraybackslash}p{\secondcolumnwidth}|>{\centering\arraybackslash}p{3.5cm}>{\centering\arraybackslash}p{5cm}|}
% \toprule
% \multirow{16}{\firstcolumnwidth}{\makecell[c]{Multimodal\\ Context\\ Modeling\\ with Memory}} & Audio Context Modeling                                                  & \multicolumn{2}{l|}{\audiocontextmodeling}                                    \\ \cline{2-4} 
%                                                          & \multirow{14}{\secondcolumnwidth}{\makecell[c]{Video Context \\Modeling}}                                 & \multicolumn{1}{l|}{Video Representation Learning}       & \videoreprlearning \\ \cline{3-4} 
%                                                          &                                                                         & \multicolumn{1}{c|}{Large Video Language Models}         & \lvlm                  \\ \cline{3-4} 
%                                                          &                                                                         & \multicolumn{1}{c|}{Video Agent}                         & \videoagent          \\ \cline{2-4} 
%                                                          & Other Modalities                                                        & \multicolumn{2}{l|}{\othermodalities}                                           \\ \hline
% \multirow{18}{\firstcolumnwidth}{\makecell[c]{Downstream \\tasks}}                        & Object-level                                                            & \multicolumn{2}{l|}{\object}                                                      \\ \cline{2-4} 
%                                                          & Action-level                                                            & \multicolumn{2}{l|}{\action}                                                      \\ \cline{2-4} 
%                                                          & General-level                                                           & \multicolumn{2}{l|}{\general}                                                     \\ \cline{2-4} 
%                                                          & Others                                                                  & \multicolumn{2}{l|}{\others}                                                      \\ \cline{2-4} 
%                                                          & Generation                                                              & \multicolumn{2}{l|}{\generation}                                                                  \\ \hline
% \multirow{14}{\firstcolumnwidth}{\makecell[c]{Multimodal \\Contextual\\ Memory for\\ Vision and\\ Robotics}}      & \makecell[c]{Multimodal \\Memory-\\Augmented \\Agents}                                      & \multicolumn{2}{l|}{\mmmemoryaugmentedagent}                                \\ \cline{2-4} 
%                                                          & \multirow{3}{\secondcolumnwidth}{\makecell[c]{Memory-\\Enhanced \\Navigation, \\Odometry, \\Manipulation}} & \multicolumn{1}{c|}{Visual Navigation}                   & \navigation            \\ \cline{3-4} 
%                                                          &                                                                         & \multicolumn{1}{c|}{Visual Odometry}                     & \odometry              \\ \cline{3-4} 
%                                                          &                                                                         & \multicolumn{1}{c|}{Manipulation Reasoning and Planning} & \manipulation          \\ \bottomrule
% \end{tabular}

\begin{tabular}{c|c|p{12.5cm}}
\toprule
\multirow{2}{*}{\makecell[c]{Multimodal\\ Context\\ Modeling\\ with Memory}} & \makecell[c]{Audio Context\\ Modeling} & Conformer-NTM \citep{DBLP:conf/interspeech/CarvalhoA23}, Loop-Copilot \citep{DBLP:journals/corr/abs-2310-12404}, MR-MT3 \citep{DBLP:journals/corr/abs-2403-10024} \\
\cmidrule{2-3}
& \multirow{3}{*}{\makecell[c]{Video Context\\ Modeling}} & \textbf{Video Representation Learning:} MC-ViT \citep{DBLP:journals/corr/abs-2402-05861}\\ 
& & \textbf{Large Video Language Models:} MovieChat \citep{DBLP:journals/corr/abs-2307-16449}, MA-LMM \citep{DBLP:journals/corr/abs-2404-05726},  VideoStreaming \citep{DBLP:journals/corr/abs-2405-16009}, 
Flash-VStream \citep{DBLP:journals/corr/abs-2406-08085}, 
VideoLLaMB \citep{wang2024videollamblongcontextvideounderstanding}, OmniDrive \citep{wang2024omnidriveholisticllmagentframework}\\ 
& & \textbf{Video Agents:} LLoVi \citep{DBLP:journals/corr/abs-2312-17235}, 
LifelongMemory \citep{DBLP:journals/corr/abs-2312-05269}, VideoAgent \citep{DBLP:journals/corr/abs-2403-10517,DBLP:journals/corr/abs-2403-11481}, ChatVideo \citep{DBLP:journals/corr/abs-2304-14407}, DoraemonGPT \citep{DBLP:journals/corr/abs-2401-08392}, LangRepo \citep{DBLP:journals/corr/abs-2403-14622}, DrVideo \citep{DBLP:journals/corr/abs-2406-12846} \\
\cmidrule{2-3}
& \makecell[c]{Other Modalities} & CSMN \citep{DBLP:conf/cvpr/ParkKK17}, DAAC \citep{DBLP:conf/iccv/HouZZXPZ21}, MGUIT \citep{DBLP:conf/cvpr/JeongKLS21}, MemoPainter \citep{DBLP:conf/cvpr/YooBCLCC19}, RMM \citep{DBLP:journals/corr/abs-2110-01033}, MM-Net \citep{DBLP:conf/iccv/WuSL021}, CDFSS \citep{DBLP:conf/cvpr/WangDWEFZ22}, MOSS \citep{DBLP:conf/cvpr/HuangYH21}, TransformerFusion \citep{DBLP:conf/nips/BozicPTDN21} \\
\midrule
\multirow{5}{*}{\makecell[c]{Downstream\\ Tasks}} & \makecell[c]{Object-level} & ConvGRU \citep{DBLP:conf/iccv/TokmakovAS17}, RFL \citep{DBLP:conf/iccvw/YangC17}, RMAN \citep{DBLP:journals/tip/PuSMZY21}, MemTrack \citep{DBLP:conf/eccv/YangC18}, STM \citep{DBLP:conf/iccv/OhLXK19}, STCN \citep{DBLP:conf/nips/ChengTT21}, STMTrack \citep{DBLP:conf/cvpr/FuLFW21}, GraphMemVOS \citep{DBLP:conf/eccv/LuWDZSG20}, DTMNet \citep{DBLP:conf/mm/ZhangWLL0L20}, TMRN \citep{DBLP:conf/iccv/SunWMZW23}, AOT \citep{DBLP:conf/nips/YangWY21}, IMANet \citep{DBLP:conf/iros/PaulDGT21}, TrackFormer \citep{DBLP:conf/cvpr/MeinhardtKLF22}, XMem \citep{DBLP:conf/eccv/ChengS22}, S-ViT \citep{DBLP:conf/cvpr/ZhaoLTCCZ23}, MMC \citep{DBLP:journals/corr/abs-2307-07812}, RFGM \citep{DBLP:conf/nips/ZhouGHL0GZ23}, RMem \citep{DBLP:journals/corr/abs-2406-08476}, MAVOS \citep{DBLP:journals/corr/abs-2403-17937}, SAM 2 \citep{ravi2024sam2segmentimages} \\
\cmidrule{2-3}
& \makecell[c]{Action-level} & LSTR \citep{DBLP:conf/nips/XuXCLXTS21}, MeMViT \citep{DBLP:conf/cvpr/WuLM0XMF22}, RViT \citep{DBLP:conf/cvpr/YangDLZSY22}, MAT \citep{DBLP:conf/iccv/WangCHWL23}, MATR \citep{song2024onlinetemporalactionlocalization} \\
\cmidrule{2-3}
& \makecell[c]{General-level} & vsLSTM \citep{DBLP:conf/eccv/ZhangCSG16}, MAVS \citep{DBLP:conf/mm/FengLKZ18}, SMN \citep{DBLP:conf/mm/Wang000FT19}, M3 \citep{DBLP:conf/cvpr/Wang000T18}, MARN \citep{DBLP:conf/cvpr/PeiZWKST19}, MART \citep{DBLP:conf/acl/LeiWSYBB20}, AAP-MIT \citep{DBLP:journals/tip/PrudvirajRVM22}, Heterogeneous Memory Enhanced Multimodal Attention Model \citep{DBLP:conf/cvpr/FanZZW0H19}, RWMN \citep{DBLP:conf/iccv/NaLKK17}, Glance-Focus \citep{DBLP:conf/nips/Bai0023} \\
\cmidrule{2-3}
& \makecell[c]{Others} & MemFlow \citep{DBLP:journals/corr/abs-2404-04808}, MAMo \citep{DBLP:conf/iccv/YasarlaCJSGP23}, MmDeblur \citep{DBLP:conf/cvpr/JiY22}, MENet \citep{DBLP:conf/eccv/SunZCCL22}, VAM \citep{DBLP:journals/tmm/KimHPR22}, MVM \citep{DBLP:conf/aaai/KimYR22} \\
\cmidrule{2-3}
& \makecell[c]{Generation} & LMC-Memory \citep{DBLP:conf/cvpr/LeeKCKR21}, MV-TON \citep{DBLP:conf/mm/ZhongWTLW21}, MemGAN \citep{Yi2020AudiodrivenTF}, SyncTalkFace \citep{DBLP:conf/aaai/ParkKHCR22}, EMMN \citep{DBLP:conf/iccv/TanJP23}, STAM \citep{DBLP:journals/tmm/00020WM023}, MemFace \citep{DBLP:journals/corr/abs-2212-05005} \\
\midrule
\multirow{3}{*}{\makecell[c]{Multimodal\\ Memory\\ for Vision\\ and Robotics}} & \makecell[c]{Memory-\\Augmented\\ Agents} & JARVIS-1 \citep{DBLP:journals/corr/abs-2311-05997}, MM-Navigator \citep{DBLP:journals/corr/abs-2311-07562}, MobileGPT \citep{DBLP:journals/corr/abs-2312-03003}, AppAgent \citep{DBLP:journals/corr/abs-2312-13771}, OS-Copilot \citep{DBLP:journals/corr/abs-2402-07456}, MEIA \citep{DBLP:journals/corr/abs-2402-00290} \\
\cmidrule{2-3}
& \makecell[c]{Memory-\\Enhanced\\ Navigation} & RPF \citep{DBLP:conf/nips/KumarGFLM18}, SSM \citep{DBLP:conf/cvpr/WangWLXS21}, VGM \citep{DBLP:conf/iccv/KwonKCYPO21}, MemoNav \citep{DBLP:journals/corr/abs-2402-19161}, SMT \citep{DBLP:conf/cvpr/FangT0S19}, MultiON \citep{DBLP:conf/nips/WaniPJCS20} \\
\cmidrule{2-3}
& \makecell[c]{Memory-\\Enhanced\\ Odometry} & Deep Visual Odometry with Adaptive Memory \citep{DBLP:journals/pami/XueWWZ22} \\
\cmidrule{2-3}
& \makecell[c]{Memory-\\Enhanced\\ Manipulation} & RDMemory \citep{DBLP:conf/icra/HuangYKPCLH24} \\
\bottomrule
\end{tabular}

% }
\end{table}
